Robust Active Distillation

Distilling knowledge from a large teacher model to a lightweight one is a widely successful approach for generating compact, powerful models in the semi-supervised learning setting where a limited amount of labeled data is available. In large-scale applications, however, the teacher tends to provide a large number of incorrect soft-labels that impairs student performance. The sheer size of the teacher additionally constrains the number of soft-labels that can be queried due to prohibitive computational and/or financial costs. The difficulty in achieving simultaneous \emph{efficiency} (i.e., minimizing soft-label queries) and \emph{robustness} (i.e., avoiding student inaccuracies due to incorrect labels) hurts the widespread application of knowledge distillation to many modern tasks. In this paper, we present a parameter-free approach with provable guarantees to query the soft-labels of points that are simultaneously informative and correctly labeled by the teacher. At the core of our work lies a game-theoretic formulation that explicitly considers the inherent trade-off between the informativeness and correctness of input instances. We establish bounds on the expected performance of our approach that hold even in worst-case distillation instances. We present empirical evaluations on popular benchmarks that demonstrate the improved distillation performance enabled by our work relative to that of state-of-the-art active learning and active distillation methods.

==> Robust Active Distillation/misc/commands.tex <==
% % Comment commands.


%                           %
%                           %
%   GENERAL      COMMANDS   %
%                           %
%                           %
\newcommand{\paragraphsmall}[1]{\textbf{{#1} $\;$}}

% \newcommand{\rev}[1]{{\color{blue}#1}}

\newcommand{\rev}[1]{{#1}}
\newcommand{\reviclr}[1]{{\color{blue}#1}}
\renewcommand{\reviclr}[1]{{#1}}
\renewcommand{\rev}[1]{{#1}}

\newcommand{\cnote}[1]{{\color{blue} (Cenk: #1)}}
\newcommand{\fnote}[1]{{\color{brown} (Fotis: #1)}}
\newcommand{\knote}[1]{{\color{red} (Khoa: #1)}}
\newcommand{\gnote}[1]{{\color{green} (Gaurav: #1)}}
\newcommand{\enote}[1]{{\color{violet} (Erik: #1)}}

% Makes comments invisible for publication-ready status. 
% COMMENT THESE LINES BELOW IF YOU WOULD LIKE TO SEE COMMENTS
\renewcommand{\cnote}[1]{}
\renewcommand{\fnote}[1]{}
\renewcommand{\knote}[1]{}
\renewcommand{\gnote}[1]{}
\renewcommand{\enote}[1]{}


\newcommand{\ignore}[1]{}


%                           %
%                           %
%   GENERAL MATH COMMANDS   %
%                           %
%                           %

\newcommand{\size}[1]{\nnz{#1}}
\newcommand{\nnz}[1]{\mathrm{nnz}(#1)}
\DeclareMathOperator*{\1}{\mathbbm{1}}
\newcommand{\compl}{\mathsf{c}}
\DeclarePairedDelimiterX{\dotp}[2]{\langle}{\rangle}{#1, #2}
\newcommand{\ramp}[1]{\left [ #1 \right]_+}

%                           %
%                           %
%   	  CONSTANTS   		%
%                           %
%                           %
\newcommand{\kmaxInsideLog}{\eta \, \eta^*}
\newcommand{\kmax}{K}
\newcommand{\kmaxSquared}{\log^2(\kmaxInsideLog)}
\newcommand{\CDef}{3 \, \kmax}
\newcommand{\LL}{\mathcal{L}}



%\newcommand{\logTermInside}[1][\eta^*]{8 \, \eta \, #1 }
\newcommand{\logTermInside}[1][4]{ \rho^* \, #1 }
\newcommand{\logTermInsideAmplif}{32 \, |\PP| \, \tau \, \eta \, \eta^* }

\newcommand{\logTermInsideGeneral}{16 \, |\PP'| \, \eta \, \eta^* }

%\newcommand{\logTerm}[1][\eta^*]{\log \left(\logTermInside[#1] / \delta \right)}
\newcommand{\logTerm}[1][\eta^*]{\log \left({#1} \, \rho^* / \delta \right)}
\newcommand{\logTermAmplif}{\log \left(\logTermInsideAmplif / \delta \right)}

\newcommand{\logTermGeneral}{\log \left(\logTermInsideGeneral / \delta \right)}

\newcommand{\kappaDef}{\sqrt{2 \lambdaStar} \left(1 + \sqrt{2 \lambdaStar} \logTerm \right)}
\newcommand{\kappaDefAmplif}{\sqrt{2 \lambdaStar} \left(1 + \sqrt{2 \lambdaStar} \logTermAmplif \right)}

\newcommand{\kappaDefGeneral}{\sqrt{2 \lambdaStar} \left(1 + \sqrt{2 \lambdaStar} \logTermGeneral \right)}

\newcommand\lambdamax{\log(\eta \, \eta^*)/2}
\newcommand{\lambdaStar}{\lambda_*}
\newcommand{\xmax}{X_\mathrm{max}}
\newcommand{\SizeOfS}[1][\rho^*]{\ceil*{\kmax' \logTerm[#1] }}

\newcommand{\SizeOfSAmplif}{\ceil*{\logTermAmplif \kmax}}

\newcommand{\SizeOfSGeneral}{\ceil*{\logTermGeneral \kmax}}


\newcommand{\tauDef}{\ceil*{\frac{\log(4 \, \eta / \delta)}{\log(10/9)}}}

\newcommand{\SizeOfT}{\ceil*{8 \log \left( 8 \, \tau \,  \eta / \, \delta\right) }}


\newcommand\BigO{\mathcal{O}}
\newcommand\Bigo{\BigO}
\newcommand\supp{\mathrm{supp}(\DD)}

\newcommand{\PRIME}[1]{#1^\prime}
\newcommand{\dotP}[2]{#1 \cdot #2}

\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}
\newcommand{\relu}[1]{\phi(#1)}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\hf}{\frac{1}{2}}
\newcommand{\dd}{{\mathrm{D}}}
\renewcommand{\AA}{{\mathcal{A}}}
\newcommand{\NN}{{\mathbb N}}
\newcommand{\iid}{\stackrel{i.i.d.}{\sim}}
\newcommand{\norm}[1]{\left\| #1\right\|}                               %
\newcommand{\br}[1]{\left\{#1\right\}}
\newcommand{\alignspace}{\qquad \qquad}

\newcommand{\abs}[1]        {\left| #1 \right|}
\newcommand{\nz}[1]{\mathrm{nz}( #1 )}
%\newcommand{\nnz}[1]{\mathrm{nnz}( #1 )}
\newcommand{\sq}{\hbox{\rlap{$\sqcap$}$\sqcup$}}
\newcommand{\eps}{\ensuremath{\varepsilon}}                       % Epsilon
\renewcommand{\epsilon}{\varepsilon}

\newcommand{\REAL}{\ensuremath{\mathbb{R}}}                       % Norm
\newcommand{\RR}{{\REAL}}
\newcommand{\margin}{{\mathrm{margin}_i}}
\newcommand{\gain}{{\mathrm{g}_i}}
\newcommand{\median}{\texttt{Median}}
\DeclareMathOperator*{\E}{\mathbb{E} \,}
\let\Pr\relax
\DeclareMathOperator*{\Pr}{\mathbb{P}}
\DeclareMathOperator*{\Var}{\text{Var}}
\newcommand{\V}{\Var}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\newcommand{\inprod}[1]{\left\langle #1 \right\rangle}
\newcommand{\eqdef}{\mathbin{\stackrel{\rm def}{=}}}
\DeclareMathOperator*{\rank}{\text{rank}}
\DeclareMathOperator*{\sign}{\text{sign}}

%                           %
%                           %
% PROJECT SPECIFIC COMMANDS %
%                           %
%                           %
\declaretheorem[name=Theorem]{theorem}
\declaretheorem[name=Corollary, numberlike=theorem]{corollary}
\declaretheorem[name=Lemma, numberlike=theorem]{lemma}
\declaretheorem[name=Proposition, numberlike=theorem]{proposition}
\declaretheorem[name=Definition]{definition}
\declaretheorem[name=Assumption]{assumption}
\declaretheorem[name=Remark, numberlike=theorem]{Remark}
\declaretheorem[name=Claim, numberlike=theorem]{Claim}
\declaretheorem[name=Example, numberlike=theorem]{Example}
\declaretheorem[name=Observation, numberlike=theorem]{Observation}

\newenvironment{itemizeAlg}{\begin{itemize}[topsep=1pt,itemsep=-1ex,partopsep=1ex,parsep=1ex]}{\end{itemize}}


\renewcommand{\index}{i}
\newcommand{\indexSet}{[s_1^\ell] \times [s_2^\ell] \times [c^\ell]}
\newcommand{\tuple}{(\tupleNoP)}
\newcommand{\tupleNoP}{h,g,r}
% In reality, the following \neuron should be the tuple index i
\newcommand{\neuron}{r}
\newcommand{\edge}{j}
\newcommand{\idx}{k}
\newcommand{\weight}{u}
\newcommand{\layers}{[L]}
\newcommand{\hiddenlayers}{[L-1]}
\newcommand{\given}{\, \mid \, }
\newcommand{\givenRealiz}{\given \realiz(\cdot), \xx}
\newcommand{\givenRealizZLemOne}{\given \xx, \EE_\ZZ}
\newcommand{\givenRealizZ}{\givenRealizZNoEps, \condGood}
\newcommand{\givenRealizZCompl}{\given \realiz(\cdot), \EE_\ZZ^\compl}

\newcommand{\condAmplif}{\EE_{\GG(\Point)}}
\newcommand{\condAmplifDef}{\EE_{\ZZ(\Point)} \cap \EE_{\Delta(\Point)}}

\newcommand{\condGood}{\EE_{\nicefrac{1}{2}}}
\newcommand{\condGoodDef}{\hat{a}(\Point) \in (1 \pm \nicefrac{1}{2}) a(\Point) \qquad \forall{\hat{a}(\cdot) \in \hat \AA^{\ell-1}}}

\newcommand{\givenAmplif}{\given \condAmplif \cap \EE^{\ell-1} }

\newcommand{\givenAmplifCompl}{\given \condAmplif^\compl \cap \EE^{\ell-1} }

\newcommand{\givenRealizSub}{\given \hat{a}^{\ell-1}(\cdot), \, \Point}

\newcommand{\realiz}{\mathbf{ a}}

\newcommand{\compressiblelayers}{[L]}
\newcommand{\etaDef}{\sum_{\ell = 1}^L \eta^\ell}
\newcommand{\etaStarDef}{\max_{\ell \in \compressiblelayers} \eta^{\ell}}

\newcommand{\ComputationTime}{\Bigo \left( \eta \, \, \eta^* \, \log \big(\eta \, \eta^*/ \delta \big) \right)}

\newcommand{\ComputationTimeGeneralized}{\Bigo \left( \eta \, \, \eta^* \, \log \big(\eta \, \eta^* \, |\PP'| / \delta \big) \right)}



\newcommand{\epsilonStar}{\epsilon_*}

\newcommand{\epsilonDenomContant}{2}
\newcommand{\epsilonPrimeDef}{\frac{\epsilon}{\epsilonDenomContant \, (L-1)}}

\newcommand{\epsilonLayer}[1][\ell]{\epsilon_{#1}}
\newcommand{\epsilonLayerDef}[1][\ell]{\frac{ \epsilon'}{ \DeltaNeuronHatLayers[#1]}}
\newcommand{\epsilonLayerDefWordy}[1][\ell]{\frac{ \epsilon}{\epsilonDenomContant \, (\LayersCompressed) \DeltaNeuronHatLayersDef[#1]}}


%\newcommand{\SampleComplexity}[1][\epsilonLayer]{\ceil*{\frac{(6 + 2\epsilon) \SNeuron \kmax \log ({{#1} / \delta}) }{\epsilon^2}}}
\newcommand{\SampleComplexity}[1][\epsilonLayer]{\ceil*{(6 + 2\epsilon) \, \SNeuron \, \kmax \, \log ({{#1} / \delta}) \epsilon^{-2}}}

\newcommand{\SampleComplexityDeltaEach}[1][\epsilonLayer]{\ceil*{\ (6 + 2{#1}) \Delta_r^2  \, \left(\sum_{\edge \in \Wpm} s_\edge\right) \, \kmax \, \log ({8 \, \eta / \delta}) \epsilon^{-2}}}

\newcommand{\SampleComplexityDelta}[1][\epsilonLayer]{(7 + 2{#1}) \Delta_r^2 \, \SNeuron_r \, \kmax \, \log ({8 \, \eta / \delta}) \epsilon^{-2}}

% \newcommand{\SampleComplexityDeltaLayers}[1][\epsilonLayer]{\ceil*{\frac{ 32  (L - 1) \, (\Delta_r^{\ell \rightarrow})^2 \left(\sum_{\edge \in \Wpm} s_\edge\right) \kmax \log ({8 \eta / \delta}) }{{#1}^2}}}
%\newcommand{\SampleComplexityDeltaLayers}[1][\epsilonLayer]{\ceil*{\frac{ 32  (L-1)  (\Delta_r^{\ell \rightarrow})^2  \kmax \log (8 \eta / \delta) \sum_{\edge \in \Wpm} s_\edge }{{#1}^2}}}

\newcommand{\SampleComplexityDeltaLayers}[1][\epsilonLayer]{\ceil*{32  \, L^2 (\Delta_r^{\ell \rightarrow})^2 \, \kmax \log (8 \eta / \delta) \,  \epsilon^{-2} \, \sum_{\edge \in \Wpm} s_\edge }}

\newcommand{\epsilonNeuron}[1][\mNeuron]{\sqrt{\frac{\tilde S}{{#1}} \left(\frac{\tilde S}{{#1}} + 6\right)} + \frac{\tilde S}{{#1}}}

\newcommand{\epsilonNeuronOpt}[1][\mNeuron]{\sqrt{\frac{\tilde S_r}{{#1}} \left(\frac{\tilde S_r}{{#1}} + 6\right)} + \frac{\tilde S_r}{{#1}}}

\newcommand{\epsilonNeuronDeterministic}[1][\mNeuron]{3 K \sum_{\edge \in (\II \setminus \II_{{#1}})} s_j}

\newcommand{\SampleComplexityWordy}{\frac{ L^2 \, (\Delta^{\ell \rightarrow})^2 \, \SNeuronWordy \, \kmax \, \log (\eta / \delta) }{\epsilon^2}}


% \newcommand{\SampleComplexityWordy}{\frac{33  \, (\LayersCompressed)^2 \, (\Delta_r^{\ell \rightarrow})^2 \, \SNeuronWordy \, \kmax \, \log (8 \, \eta / \delta) }{\epsilon^2}}

\newcommand{\SampleComplexityGeneral}{\ceil*{\frac{32  \, (\LayersCompressed)^2 \, (\DeltaNeuronHatLayers)^2 \, \SNeuronWordy \, \kmax \, \log (16 \, |\PP'| \, \eta / \delta) }{\epsilon^2}}}

\newcommand{\SampleComplexityGeneralConcise}[1][\epsilonLayer]{\ceil*{\frac{8  \, \SNeuron \, \kmax \log ({16  |\PP'| \, \eta / \delta}) }{{#1}^2}}}

\newcommand{\SampleComplexityAmplif}[1][\epsilonLayer]{\ceil*{\frac{8  \, \SNeuron \, \kmax \log ({32  |\PP| \, \tau \, \eta / \delta}) }{{#1}^2}}}


\newcommand{\LayersCompressed}{L}
\newcommand{\epsilonPrime}{\frac{\epsilon}{2 \, (\LayersCompressed)}}

\newcommand{\param}{\theta}
\newcommand{\paramDef}{(\WW^1, \ldots, \WW^L)}
\newcommand{\paramHat}{\hat{\theta}}
\newcommand{\paramHatDef}{(\WWHat^1, \ldots, \WWHat^L)}

\newcommand{\ComputationTimeSum}[1]{\sum_{\ell = #1}^L \eta^{\ell-1} \eta^{\ell}}

\newcommand{\f}{f_\param}
\newcommand{\fHat}{f_{\paramHat}}

\newcommand{\Input}{x}
\newcommand{\Label}{y}
\newcommand{\Point}{\Input}
\newcommand{\PointPrime}{\Input'}
\newcommand{\xx}{\mathbf{\Input}}

\newcommand{\pos}{\mathrm{pos}}
\newcommand{\negg}{\mathrm{neg}}
\newcommand{\InputPos}{\Input_\pos}
\newcommand{\InputNeg}{\Input_\mathrm{neg}}


\newcommand{\Wpm}{\II}
\newcommand{\Wplus}{\II_+}
\newcommand{\Wminus}{\II_-}
\newcommand{\WplusDefVerbose}{\{\edge \in  \II : w_\edge > 0\}}
\newcommand{\WminusDefVerbose}{\{\edge \in  \II: w_\edge < 0 \}}
\newcommand{\WplusDef}{\WplusDefVerbose}
\newcommand{\WminusDef}{\WminusDefVerbose}


\newcommand{\II}{\mathcal{I}}

% \newcommand{\gDef}[1]{\max_{a(\cdot) \in \AA^{\ell-1}} \, \frac{\WWRowCon_\edge \, a_{\edge}(#1)}{\sum_{\idx \in \II } \WWRowCon_\idx \, a_{\idx}(#1) }}
\newcommand{\gDefNoMax}[2][a]{ \frac{\WWRowCon_\edge \, {#1}_{\edge}(#2)}{\sum_{\idx \in \II } \WWRowCon_\idx \, {#1}_{\idx}(#2) }}
\newcommand{\gDefNoMaxNice}[2][a]{ \nicefrac{\WWRowCon_\edge \, {#1}_{\edge}(#2)}{\sum_{\idx \in \II } \WWRowCon_\idx \, {#1}_{\idx}(#2) }}

\newcommand{\gDef}[2][a]{\max_{{#1}(\cdot) \in \AA} \gDefNoMax[{#1}]{#2}}
\newcommand{\gDefNice}[2][a]{\max_{{#1}(\cdot) \in \AA} \gDefNoMaxNice[{#1}]{#2}}

\newcommand{\gHatDef}[1]{\max_{a(\cdot) \in \AA^{\ell-1}} \, \frac{\WWRowCon_\edge \, \hat a_{\edge}(#1)}{\sum_{\idx \in \II} \WWRowCon_\idx \, \hat a_{\idx}(#1) }}


\newcommand{\cdf}[1]{F_\edge \left(#1 \right)}
\newcommand{\cdfHat}[1]{\hat F_\edge \left(#1 \right)}


% for pseudo-code only
\newcommand{\sPM}[1][\edge]{s_{#1}}
\newcommand{\mPM}{m}
\newcommand{\qPM}[1]{q_{#1}}


\newcommand{\mNeuron}{m}
\newcommand{\mNeuronWordy}{\mNeuron_r}
\newcommand{\mPos}{m^+_\neuron}
\newcommand{\mNeg}{m^-_\neuron}
\newcommand{\SNeuron}{S}
\newcommand{\SNeuronWordy}{S_\neuron^\ell}
%\newcommand{\STildeDef}[1][]{\SNeuron_{{#}} \kmax \log ({8 \, \eta / \delta)}}
%\newcommand{\STildeDef}[1][]{\SNeuron_{{r}} \kmax \log ({{#1} / \delta)}}
\newcommand{\STildeDef}[2][]{\SNeuron_{{#1}} \kmax \log ({{#2} / \delta)}}
\newcommand{\SPos}{\SNeuronWordy{^+}}
\newcommand{\SNeg}{\SNeuronWordy{^-}}
\renewcommand{\S}{S}

\newcommand{\T}[1][]{T_{#1}}
\newcommand{\TTilde}[1][]{\widetilde{T}_{#1}}
\newcommand{\TMinTilde}[1][]{\tilde{T}^-_{#1}}

\newcommand{\bound}{M}


\newcommand{\WWRow}[1][\neuron]{w_{#1}}
\newcommand{\WWHatRow}[1][\neuron]{{\hat{w}_{#1}}}
\newcommand{\WWRowCon}[1][\neuron]{w}
\newcommand{\WWHatRowCon}[1][\neuron]{{\hat{w}}}
\newcommand{\WWHat}{\hat{\WW}}
\newcommand{\student}{\theta_\mathrm{student}}
\newcommand{\teacher}{\theta_\mathrm{teacher}}


\newcommand{\alglinelabel}{%
  \addtocounter{ALC@line}{-1}% Reduce line counter by 1
  \refstepcounter{ALC@line}% Increment line counter with reference capability
  \label% Regular \label
}


\newcommandx*{\w}[1][1=x]{w_{a,b}(#1)}
\newcommandx*{\ws}[1][1=x]{w(#1)}

\newcommandx*{\g}[1][1=x]{g_{a,b}(#1)}
\newcommandx*{\gPrime}[1][1=x]{g'_{a,b}(#1)}
\newcommandx*{\gDPrime}[1][1=x]{g''_{a,b}(#1)}
\newcommandx*{\h}[1][1=x]{h_{a,b}(#1)}
\newcommandx*{\hPrime}[1][1=x]{h'_{a,b}(#1)}
\newcommand{\rh}{\hat r_t}

\newcommand{\DeltaNeuronTrue}{\Delta_\index^{\ell}}
\newcommand{\DeltaNeuronDef}[1][{\Point}]{\frac{z_\index^+(#1) + z_\index^-(#1)}{|z_\index(#1)|}}

\newcommand{\DeltaNeuronTrueDef}[1][\xx]{ \frac{\sum_{\idx \in [\eta^{\ell-1}]}  |\WWRow[\neuron \idx]^\ell \, a_\idx^{\ell-1}(#1)|} {\left|\sum_{\idx \in [\eta^{\ell-1}]} \WWRow[\neuron \idx]^\ell \, a_\idx^{\ell-1}({#1})\right|}}


\newcommand{\Wpl}{\Wplus}
\newcommand{\Wmi}{\Wminus}
\newcommand{\s}[1][\edge]{s_{#1}}


\newcommand{\SPlu}{S_+}
\newcommand{\SMin}{S_-}
\newcommand{\CC}{\mathcal C}
\newcommand{\SNeu}{S^{\ell}_\neuron}

\newcommand{\G}{\Gamma}
\newcommand{\DD}{{\mathcal D}}
\newcommand{\QQ}{{\mathbb Q}}
\newcommand{\ZZ}{{\mathcal Z}}

\newcommand{\FF}{{\mathcal F}}
\newcommand{\XX}{\mathcal{X}}
\newcommand{\EE}{\mathcal{E}}
\newcommand{\YY}{\mathcal{Y}}
\newcommand{\WW}{W}


% % Expectation with respect to coreset C
\newcommand{\EPlu}{\E \nolimits_{\CC \given \hat a(\cdot), \, \Point}\,}

% % Variance with respect to coreset C
\newcommand{\VarCond}{\Var \nolimits_{\CC \given \hat a(\cdot), \, \Point}\, }

% % Expectation with respect to coreset C
\newcommand{\EPluLemOne}{\E \nolimits_{\CC \givenRealizZLemOne}\,}

% % Variance with respect to coreset C
\newcommand{\VarCondLemOne}{\Var \nolimits_{\CC \givenRealizZLemOne}\, }

\newcommand\Reals{\mathbb{R}}
\newcommand\PP{\mathcal{P}}
\renewcommand\QQ{\mathcal{Q}}
\renewcommand\SS{\mathcal{S}}
\newcommand\MM{\mathcal{M}}
\newcommand\LLL{\mathcal{L}}
\newcommand\GG{\mathcal{G}}
\newcommand\TT{\mathcal{T}}
\newcommand\VV{\mathcal{V}}
\newcommand\BB{\mathcal{B}}

\DefineFNsymbols{mySymbols}{{\ensuremath\dagger}  {\ensuremath\ddagger} *\P
   *{**}{\ensuremath{\dagger\dagger}}{\ensuremath{\ddagger\ddagger}}}
\setfnsymbol{mySymbols}

\renewcommand\cite{\citep}

% \usepackage[shortlabels]{enumitem}
% % \setlist{nolistsep, noitemsep,leftmargin=12pt, labelwidth=1pt, topsep=0pt, partopsep=0pt}
% \setlist{leftmargin=12pt, labelwidth=1pt, topsep=0pt, partopsep=0pt}
% \captionsetup{belowskip=0pt}



==> Robust Active Distillation/misc/preamble.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{nicefrac}
\usepackage{wrapfig}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage[export]{adjustbox}
\usepackage{subcaption}

\usepackage{float} 
\usepackage[bookmarks=true,backref=page,colorlinks=true,allcolors=blue]{hyperref}
\usepackage{amsmath,amsfonts,amsthm,amssymb, nccmath}
\allowdisplaybreaks % allow page breaks of equations
\usepackage{bbm}
\usepackage{framed}
\usepackage{enumerate}
\usepackage{mathtools}
%\usepackage{scalefnt}
\usepackage{changepage}
\usepackage{xargs}


\usepackage{natbib}
% I'm adding new packages
\usepackage{comment}
\usepackage{setspace}
\usepackage{verbatim}
\usepackage{xcolor}
\usepackage[font=small]{caption}
\usepackage{scalefnt}
\usepackage{xr}
\usepackage[shortlabels]{enumitem}
\usepackage{placeins}
\usepackage{color}
\usepackage{footmisc}
\usepackage{nicefrac}

\usepackage{thmtools}
\usepackage{thm-restate}
\usepackage{multirow}
\usepackage{amsfonts}
\usepackage{bbm}

==> Robust Active Distillation/sec/abstract.tex <==
\begin{abstract}

 Distilling knowledge from a large teacher model to a lightweight one is a widely successful approach for generating compact, powerful models in the semi-supervised learning setting where a limited amount of labeled data is available. In large-scale applications, however, the teacher tends to provide a large number of incorrect soft-labels that impairs student performance. The sheer size of the teacher additionally constrains the number of soft-labels that can be queried due to prohibitive computational and/or financial costs. The difficulty in achieving simultaneous \emph{efficiency} (i.e., minimizing soft-label queries) and \emph{robustness} (i.e., avoiding student inaccuracies due to incorrect labels) hurts the widespread application of knowledge distillation to many modern tasks. In this paper, we present a parameter-free approach with provable guarantees to query the soft-labels of points that are simultaneously informative and correctly labeled by the teacher. At the core of our work lies a game-theoretic formulation that explicitly considers the inherent trade-off between the informativeness and correctness of input instances. We establish bounds on the expected performance of our approach that hold even in worst-case distillation instances. We present empirical evaluations on popular benchmarks that demonstrate the improved distillation performance enabled by our work relative to that of state-of-the-art active learning and active distillation methods.
%We present empirical evaluations on benchmark scenarios that demonstrate the effectiveness of our work in generating high-quality student models in a fast and reliable way.

% The success of knowledge distillation largely hinges on generating \emph{correct} teacher soft-labels to teach the student in an \emph{efficient} way. %Soft-labels that are not in agreement with the groundtruth label lead to poor student performance due to misguided training. On other hand, if the mo

\end{abstract}

==> Robust Active Distillation/sec/analysis.tex <==
\section{Analysis}
\label{sec:analysis}

We assume throughout that $\nnz{g} > m$ so that the optimal objective value of \eqref{eqn:problem} is strictly positive. 
\begin{lemma}
An optimal solution $p^* \in \Delta$ to \eqref{eqn:problem} has $k$ non-zero entries $\II_k \subseteq [n]$ corresponding to the $k$ indices of the largest entries of $g$, with
$$
p^*_i = \frac{1}{g_i \sum_{j \in \II_k} g_j^{-1}} \quad \forall{i \in \II_k},
$$
with objective value
$$
\frac{k - m}{ \sum_{j \in \II_k} g_j^{-1}}.
$$
The distribution $p^*$ can be computed in $\Theta(n \log n)$ time.
\end{lemma} 
\begin{proof}
Let $p$ be an optimal solution to \eqref{eqn:problem} and WLOG assume that $p_1 g_1 \ge p_2 g_2 \ge \cdots p_n g_n$. Let $k = \nnz{p}$ and define $S(p, g) = \sum_{i = m+1}^k p_i g_i$. Note that 
$$
S(p, g) = \min_{c \in \{0, 1\}^n: \dotp{c}{\mathbf{1}} = n - m} \E \nolimits_{i \sim p}[g_i c_i]
$$
since the adversary would select $c$ to remove the top $m$ highest entries of $p g$.

Let $w = p_{m+1} g_{m+1}$. By optimality of $p$, it must be that $p_1 g_1 = \cdots = p_{m+1} g_{m+1} = w$. Otherwise, we could increase the value of $p_{m+1} g_{m+1}$ by removing probability mass from $p_1, \ldots, p_m$ and increasing $p_{m+1}$ accordingly until $pg$ is equal in the first $m+1$ entries, which would lead to a higher objective value.

We now claim that in fact $p_1 g_1 = \cdots = p_k g_k$ for some optimal $p$. Suppose this does not hold, i.e., the equality in probability-weighted gains are not equal for all optimal solutions.  optimal solution $p$ smallest index $j > m+1$ for which $p_j g_j < w$. Construct a new probability distribution $p'$ by scaling up the probabilities $p_j, \ldots, p_k$ by $\alpha > 1$ and scaling down $p_1, \ldots, p_{j-1}$ by $\beta \in (0,1)$ until $p_j g_j$ matches the rescaled $w$, i.e., $\alpha p_j g_j = \beta w = \beta p_{m+1} g_{m+1}$. The values for $\alpha$ and $\beta$ that lead to such a probability distribution are
$$
\alpha = \frac{w}{(1 - z) p_j g_j + z w} \quad \text{and} \quad \beta = 1 - \frac{z(\alpha - 1)}{1 - z},
$$
where $z = \sum_{i = j}^k p_i$. Note that $p'$ is indeed a valid distribution since the sum is equal to 1 and none of the increased probabilities exceed 1\footnote{Since $
\alpha p_i = \frac{w p_i}{(1 - z) p_j g_j + z w} \leq \frac{zw}{(1 - z) p_j g_j + z w} \leq 1
$ for all $i = j, \ldots, k$.}.


Define $S_1 = \sum_{i=j}^{k} p_i g_i$ and $S_2 = \sum_{i=1}^{j-1} p_i g_i$ and note that $S(p, g) = S_1 + S_2$. Similarly, for $p'$ defined as the rescaled distribution above, we have $S(p', g) = \alpha S_1 + \beta S_2$. We now compare $S(p', g)$ and $S(p, g)$:
\begin{align*}
    S(p', g) - S(p, g) &= \alpha S_1 + \beta S_2 - (S_1 + S_2) \\
    %&= (\alpha - 1) S_1 - \frac{z(\alpha - 1) S_2}{1 - z} \\
    &= (\alpha - 1) \left(S_1 - \frac{z}{1-z} S_2\right).
\end{align*}
It follows that $(\alpha - 1) > 0$ by definition, so the quantity above is strictly positive if $S_1 > \frac{z}{1-z} S_2$. By the optimality of $p$, we know that it is better to have the entries of $j, \ldots, k$ to be non-zero. This means that if we were to set $p_j, \ldots, p_k$ to 0 and increase the probabilities $p_1, \ldots, p_{j-1}$ by a factor of $(1 - z)^{-1}$, we would have a lower objective value\footnote{If the objective values are equal, then we are done since the altered probability distribution is an optimal solution with $j$ non-zero entries $p_1 g_1 = \cdots = p_j g_j$.}.
%\footnote{If the objective value is the same, i.e., if $p$ is not a unique solution, then we can recurse on this argument by starting from the rescaled distribution with $p_j, \ldots, p_k = 0$ until an optimal solution with fewer nonzero entries is not possible.}
$$
S_1 + S_2 > \frac{S_2}{1-z}.
$$
Rearranging, this implies that $S_1 > z/(1-z) S_2$, and from the calculations above, that
$$
S(p', g) - S(p, g) > 0,
$$
which contradicts the optimality of $p$. This proves that the optimal distribution $p$ must satisfy 
$$
p_{i} g_{i} = p_{j} g_{j} \quad \forall{i, j \in \nz{p}},
$$
where $\nz{p} = \{i \in [n] : p_i > 0 \}$.

To complete the proof, note that the above means that the optimal distribution $p$ must have the form
\begin{equation}
\label{eqn:closed-form}
p_i = \frac{1}{g_i \sum_{j \in \nz{p}} g_j^{-1}} \quad \forall{i \in \nz{p}},
\end{equation}
with the objective value 
\begin{equation}
\label{eqn:obj-val}
\frac{|\nz{p}| - m}{\sum_{j \in \nz{p}} g_j^{-1}}.
\end{equation}
For a fixed $\nnz{p}$, the above is maximized whenever $\sum_{j \in \nz{p}} g_j^{-1}$ is minimized, which occurs when the indices of non-zero probabilities $\nz{p}$ correspond to the top-$|\nz{p}|$ gains. The optimal distribution can be generated as follows. First, we sort the gains in descending order $g_1 \ge g_2 \ge \cdots \ge g_n$ and pre-compute the cumulative histogram for $\sum_{j =1}^k g_j^{-1}$ for each $k \in [n]$. This takes $\Theta(n \log n)$ time. Then, we generate $\nz{p}$ by picking the $k \in [n]$ that maximizes \eqref{eqn:obj-val}. This takes $\Theta(n)$ time, for a total of $\Theta(n \log n)$ time to generate $p^*$.

% At each iteration $i \in [n]$, we check whether setting the $i^\text{th}$ index as in Eq.~\ref{eqn:closed-form} would lead to an increase in the objective value and if so, we set it accordingly, otherwise we stop and return the probability vector. From the objective value above, we see that the stopping condition occurs when
% $$
% \frac{|\nz{p}| + 1 - m}{\sum_{j \in \nz{p}} g_j^{-1} + g_i^{-1}} < \frac{|\nz{p}| - m}{\sum_{j \in \nz{p}} g_j^{-1}}
% $$
\end{proof}

\subsection{Batch-based Formulation}
\newtheorem{observation}[theorem]{Observation}
\begin{observation}[Diminishing returns]
The rate of gain $r_i$ of each bucket $i \in [t]$ is monotonically decreasing with the amount of mass allotted to it, i.e.,
$r_i(x) \leq r_i(y)$ for $x \ge y$.
\end{observation}

\begin{lemma}[Monotonicity of optimal allocation]
Let $\AA^*(b) = (b_1, ..., b_t)$ with $\sum_{i=1}^t \AA_i^*(b) = b$ be the optimal allocation with respect to budget b. For any $b' \geq b$, we have that $\AA^*_i(b) \leq \AA^*_i(b')$ for all $i \in [t]$.
\end{lemma}
\begin{proof}
Suppose there exists $i \in [t]$ such that $\AA^*_i(b) > \AA^*_i(b')$. This implies that there must exist a $j \in [t]$ such that $\AA^*_j(b) < \AA^*_j(b')$ with 
\begin{equation}
\label{eqn:exists}
r_i(\AA^*_i(b')) < r_j(\AA^*_j(b') - \epsilon)
\end{equation}
for all $\epsilon \in (0, \AA^*_j(b')]$. But, by Observation 1 and the fact that $\AA^*_i(b)$ is optimal for budget $b$, we observe a contradiction for $\epsilon = \min\{\AA^*_i(b) - \AA^*_i(b'),\AA^*_j(b') - \AA^*_j(b)\}$:
\begin{align*}
r_i(\AA^*_i(b')) &\ge r_i(\AA^*_i(b) - \epsilon) &\text{by Observation 1 since $\AA^*_i(b') \leq \AA^*_i(b) - \epsilon$} \\
&\ge r_j(\AA^*_j(b)) &\text{By optimality of $\AA^*(b)$}\\
&\ge r_j(\AA^*_j(b') - \epsilon) &\text{by Observation 1 since $\AA^*_j(b) \leq \AA^*_j(b') - \epsilon$} \\
&> r_i(\AA^*_i(b')) &\text{by \eqref{eqn:exists}},
\end{align*}
and this establishes the lemma.
\end{proof}

==> Robust Active Distillation/sec/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
% In this paper, we considered the problem of efficient and robust knowledge distillation in the semi-supervised learning setting with a limited amount of labeled data and a large amount of unlabeled data. We formulated the problem of robust active distillation and presented a near linear-time algorithm with provable guarantees to solve it optimally. To the best of our knowledge, our work is the first is to first to consider importance sampling for informative and correctly labeled soft-labels to enable efficiency and robustness in large-scale knowledge distillation tasks. Our method is parameter-free and simple-to-implement. Our experiments on popular benchmark data sets with a diverse set of configurations showed a consistent and notable improvement in the test accuracy of the generated student model relative to those generated by state-of-the-art methods. We envision that our approach can be used to generate lightweight, high-performance student models by distilling the knowledge of large, bulky models in the face of limited amount of labeled data. 


In this paper, we considered the problem of efficient and robust knowledge distillation in the semi-supervised learning setting with a limited amount of labeled data and a large amount of unlabeled data. We formulated the problem of robust active distillation and presented a near linear-time algorithm with provable guarantees to solve it optimally. To the best of our knowledge, our work is the first to consider importance sampling for informative and correctly labeled soft-labels to enable efficiency and robustness in large-scale knowledge distillation tasks. Our method is parameter-free and simple-to-implement. Our experiments on popular benchmark data sets with a diverse set of configurations showed a consistent and notable improvement in the test accuracy of the generated student model relative to those generated by state-of-the-art methods. 

\paragraph{Limitations and future work} In future work, we plan to establish a deeper theoretical understanding on the trade-offs of the various instantiations of our general framework, \eqref{prb:ours-general} in Sec.~\ref{sec:rad}, on the \emph{test accuracy} of the student model. For example, it is not clear whether defining the gain as $\gain= 1 - \margin$ or $\gain = \exp(-\margin)$ is more appropriate, even though both definitions lead to gains that are monotonically increasing with the uncertainty of the student. Besides considering teacher accuracy in the robust formulation, we plan to also consider other relevant metrics such as student-teacher disagreement to construct more informed distributions. Overall, we envision that our approach can be used in high-impact applications to generate powerful student models by efficiently distilling the knowledge of large teachers in the face of limited labeled data.

%Relatedly, we conjecture that there exists a closed-form solution for the more challenging problem of minimizing the \emph{performance gap} with respect to the best sampling distribution in hindsight -- this is akin to regret bounds in online learning.
%For future work, we plan to refine our robust active distillation formulation and extend it to the batch sampling setting. For example, it could be 



==> Robust Active Distillation/sec/introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Deep neural network models have been unprecedentedly successful in many high-impact application areas such as Natural Language Processing~\citep{ramesh2021zero,brown2020language} and Computer Vision~\citep{ramesh2021zero,niemeyer2021giraffe}. However, this has come at the cost of using increasingly large labeled data sets and high-capacity network models that tend to contain billions of parameters~\citep{devlin2018bert}. These models are often prohibitively costly to use for inference and require millions of dollars in compute to train~\citep{patterson2021carbon}. Their sheer size also precludes their use in time-critical applications where fast decisions have to be made, e.g., autonomous driving, and deployment to resource-constrained platforms, e.g., mobile phones and small embedded systems~\citep{baykal2022sensitivity}. To alleviate these issues, a vast amount of recent work in machine learning has focused on methods to generate compact, powerful network models without the need for massive labeled data sets.


Knowledge Distillation (KD)~\citep{bucilua2006model, hinton2015distilling, gou2021knowledge,beyer2021knowledge} is a general purpose approach that has shown promise in generating lightweight powerful models even when a limited amount of labeled data is available~\citep{chen2020big}. The key idea is to use a large teacher model trained on labeled examples to train a compact student model so that its predictions imitate those of the teacher. The premise is that even a small student is capable enough to \emph{represent} complicated solutions, even though it may lack the inductive biases to appropriately learn representations from limited data on its own~\citep{stanton2021does,menon2020distillation}. In practice, KD often leads to significantly more predictive models than otherwise possible with training in isolation~\citep{chen2020big,xie2020self,gou2021knowledge,cho2019efficacy}.

Knowledge Distillation has recently been used to obtain state-of-the-art results in the semi-supervised setting where a small number of labeled and a large number of unlabeled examples are available~\citep{chen2020big,pham2021meta,xie2020self}. \emph{Semi-supervised KD} entails training a teacher model on the labeled set and using its soft labels on the unlabeled data to train the student. The teacher is often a pre-trained model and may also be a generic large model such as GPT-3~\cite{brown2020language} or PaLM~\cite{chowdhery2022palm}. The premise is that a large teacher model can more aptly extract knowledge and learn from a labeled data set, which can subsequently be distilled into a small student. %by using the teacher’s soft labels on the unlabeled data. 
%using self-supervised learning techniques.}


% Knowledge Distillation (KD)~\cite{bucilua2006model, hinton2015distilling, gou2021knowledge,beyer2021knowledge} is a general purpose approach that has shown promise in generating lightweight powerful models even when a limited amount of labeled data is available~\cite{chen2020big}. The key idea is to use a large teacher model trained on labeled examples to train a compact student model so that its predictions imitate those of the teacher. In the semi-supervised setting where a small number of labeled and a large number of unlabeled examples are available, this entails training the teacher model on the labeled set and using the teacher's soft labels on the unlabeled data to train the student. The premise of KD is that even a small student is capable enough to \emph{represent} complicated solutions, even though it may lack the inductive biases to appropriately learn representations from limited data on its own~\cite{stanton2021does,menon2020distillation}. In practice, KD often leads to significantly more predictive models than otherwise possible with training in isolation~\cite{chen2020big,xie2020self,gou2021knowledge,cho2019efficacy}.

Despite its widespread success, KD generally suffers from various degrees of \emph{confirmation bias} and \emph{inefficiency} in modern applications to semi-supervised learning. Confirmation bias~\cite{pham2021meta,liu2021certainty,arazo2020pseudo,beyer2021knowledge} is the phenomenon where the student exhibits poor performance due to training on noisy or inaccurate teacher soft-labels. Here, inaccuracy refers to the inconsistency between the teacher's predictions for the unlabeled inputs and their groundtruth labels. Feeding the student inaccurate soft-labels leads to increased confidence in incorrect predictions, which consequently produces a model that tends to resist new changes and perform poorly overall~\cite{liu2021certainty,arazo2020pseudo}. At the same time, large-scale applications often require the teacher's predictions for billions of unlabeled points. \rev{For instance, consider distilling knowledge from GPT-3 to train a powerful student model. As of this writing, OpenAI charges 6c per 1k token predictions~\citep{OpenAIpricing}. Assuming just 1M examples to label and an average of 100 tokens per example leads to a total cost of $\$6$M. Hence, it is highly desirable to acquire the most helpful -- i.e., informative and correct -- soft-labels subject to a labeling budget (GPT-3 API calls) to obtain the most powerful student model for the target application.}

%Hence, it is highly desirable to minimize the number of API calls to GPT-3 (softlabels) in order to minimize the distillation cost


% it is imperative that we only a portion of the large unlabeled data set is 

% A prominent challenge in applying KD in the semi-supervised setting is that the teacher's predictions for the unlabeled inputs may be inaccurate with respect to the ground-truth label or misleading altogether for the student. This is known as the problem of confirmation 

 %In this paper, we consider the problem of query-efficient and robust active distillation to remedy the issues of confirmation bias and inefficiency in modern large-scale knowledge distillation applications. 
 
%  In this paper, we consider the problem of \emph{efficient} and \emph{robust} large-scale knowledge distillation in the semi-supervised setting where a small number of labeled and a large number of unlabeled examples are available.
 
 Thus, it has become increasingly important to develop KD methods that are both query-efficient and robust to labeling inaccuracies.
 Prior work in this realm is limited to tackling \emph{either} distillation efficiency~\cite{liang2022few,xu2020computation}, by combining mix-up~\cite{zhang2017mixup} and uncertainty-based sampling~\cite{roth2006margin}, or robustness~\cite{pham2021meta,liu2021certainty,arazo2020pseudo,zheng2021meta,zhang2020distilling}, through clever training and weighting strategies, but \rev{\emph{not both of these objectives at the same time}}. In this paper, we present a simple-to-implement method that finds a sweet spot and improves over standard techniques. \rev{Relatedly, there has been prior work in learning under label noise (see  \citet{song2022learning} for a survey), however, these works generally assume that the noisy labels are available (i.e., no active learning component) or impose assumptions on the type of label noise~\cite{younesian2021qactor}. In contrast, we assume that the label noise can be fully adversarial and that we do not have full access to even the noisy labels.}
 
 %In this paper, we show that this is a particularly challenging problem because efficiency (i.e., minimizing soft-label queries) and robustness (i.e., training on correct soft-labels) are competing objectives that require delicate and explicit consideration.


To the best of our knowledge, this work is the first to consider the problem of importance sampling for simultaneous efficiency and robustness in knowledge distillation. To bridge this research gap, we present an efficient algorithm with provable guarantees to identify unlabeled points with soft-labels that tend to be simultaneously informative and accurate. Our approach is parameter-free, imposes no assumptions on the problem setting, and can be widely applied to any  network architecture and data set. At its core lies the formulation of an optimization problem that simultaneously captures the objectives of efficiency and robustness in an appropriate way. In particular, this paper contributes:
\rev{
\begin{enumerate}
    \item A mathematical problem formulation that captures the joint objective of training on \emph{informative} soft-labels that are accurately labeled by the teacher in a query-efficient way
    \item A near linear time, parameter-free algorithm to optimally solve it
    \item Empirical results on benchmark data sets and architectures with varying configurations that demonstrate the improved effectiveness of our approach relative to
    the state-of-the-art
    \item Extensive empirical evaluations that support the widespread applicability and robustness of our approach to varying scenarios and practitioner-imposed constraints.
\end{enumerate}
}
% In this paper, we consider the problem of \emph{efficient} and \emph{robust} large-scale knowledge distillation in the semi-supervised setting where a small number of labeled and a large number of unlabeled examples are available. Prior work in this realm is limited to tackling \emph{either} distillation efficiency~\cite{liang2022few,xu2020computation}, by combining mix-up~\cite{zhang2017mixup} and uncertainty-based sampling~\cite{roth2006margin}, or robustness~\cite{pham2021meta,liu2021certainty,arazo2020pseudo,zheng2021meta,zhang2020distilling}, through clever training and weighting strategies, but not both of these objectives at the same time in selecting the appropriate points to soft-label. In this paper, we show that this is a particularly challenging problem because efficiency (i.e., minimizing soft-label queries) and robustness (i.e., training on correct soft-labels) are competing objectives that require delicate and explicit consideration.

% To the best of our knowledge, this work is the first to consider the problem of importance sampling for simultaneous efficiency and robustness in knowledge distillation. To bridge this research gap, we present an efficient algorithm with provable guarantees to identify unlabeled points with soft-labels that tend to be simultaneously informative and accurate. Our approach is parameter-free, imposes no assumptions on the problem setting, and can be widely applied to any  network architecture and data set. At the core of our method lies the formulation of an optimization problem that simultaneously captures the objectives of efficiency and robustness in an appropriate way.


% In this paper, we consider the problem of \emph{efficient} and \emph{robust} large-scale knowledge distillation in the semi-supervised setting where a small number of labeled and a large number of unlabeled examples are available. To this end, we present an efficient, parameter-free algorithm with provable guarantees to query the soft-labels of a \emph{small} set of points that tend to be simultaneously informative and accurate. Our approach imposes no assumptions on the problem setting and can be widely applied to any student-and-teacher architecture combination and any data set. At the core of our work lies the formulation of an optimization problem that simultaneously captures the objectives of data efficiency and soft-label accuracy in an appropriate way.

%Our work aims to advance knowledge efficient and robust knowledge distillation that can be widely applied to large-scale data sets and network architectures. In particular, we:
% \begin{enumerate}
%     \item A mathematical problem formulation for the joint objective of querying \emph{informative} soft-labels that tend to be accurate in a data-efficient way
%     \item A near linear time, parameter-free algorithm to optimally solve it
%     \item Empirical results on benchmark data sets and network architectures that demonstrate the improved effectiveness of our approach relative to state-of-the-art.
% \end{enumerate}






==> Robust Active Distillation/sec/method.tex <==
% \section{Pseudocode to be moved somewhere}
% \label{sec:method}

\begin{algorithm}
\small
\caption{\textsc{ActiveDistillation}}
\label{alg:active-distillation}
\textbf{Input:} a set of labeled points $(\XX_L, \YY_L)$, a set of unlabeled points $\XX_U$, the number of points to soft-label per iteration $b \in \mathbb{N}_+$, and a selection algorithm \textsc{Select}$(\bar \XX, \theta, b)$ that selects a sample of size $b$ from $\bar \XX$
\begin{spacing}{1}
\begin{algorithmic}[1]
\small
\STATE $\mathcal{P} \gets (\XX_L, \YY_L)$; \COMMENT{Training set thus far; initially only hard-labeled points} \\
\STATE $\teacher \gets \textsc{Train}(\PP, \teacher^{\mathrm{random}});$ \COMMENT{Train teacher on labeled data starting from random initialization}
\STATE $\theta_0 \gets \textsc{Train}(\PP, \student^{\mathrm{random}});$ \COMMENT{Train student on labeled data starting from random initialization}
\STATE $\SS \gets \emptyset;$ \COMMENT{Set of inputs that have been soft-labeled} \\
\FOR{$t \in \{1, \ldots, T\}$} \label{lin:start-active}
    %\STATE $\SS_t \gets \textsc{Select}(\XX_B \setminus \SS, \theta_{t-1}, b)$ \COMMENT{Select $b$ points to be soft-labeled by $\teacher$} \label{lin:select} \\
    \STATE $\SS_t \gets \textsc{Select}(\XX_U \setminus \SS, \theta_{t-1}, b)$ \COMMENT{Select $b$ points to be soft-labeled by $\teacher$} \label{lin:select} \\
    \STATE $\SS \gets \SS \cup \SS_t$ \COMMENT{Add new points so we do not sample them again}  \\
    \STATE $\PP \gets \PP \cup \{\left(x, f_{\teacher}(x)\right) : x \in \SS_t \}$ \label{lin:soft-label} \COMMENT{Soft-label points and add them to the training set} \\ 
    %\STATE (\text{if \textbf{rand-init} option} $\theta_{t-1} \gets \textsc{RandomInitStudentNetwork()}$)
    \STATE $\theta_t \gets \textsc{Train}(\PP, \theta_\mathrm{student}^\mathrm{random})$ \COMMENT{Train network with the additional soft-labeled points from scratch} \label{lin:train}
\ENDFOR \label{lin:end-active}
\STATE \textbf{return} $\theta_T$
\end{algorithmic}
\end{spacing}
\end{algorithm}

==> Robust Active Distillation/sec/minimax.tex <==

% \section{Proof for relative penalties}
% \enote{This should be replaced with the previous section, ``Proof for general penalties.''}

% \begin{lemma}
% \label{lem:minimax-max-gain-old}
% Let $n > m$ be integers, together with weight $w \ge 0$, such that $n-m(1+w) \ge 0$.
% Let $f(p, c) = \sum_i g_i p_i c_i - \sum_i w g_i p_i (1-c_i)$, and let $\Delta_{\ell} = \{ x\in [0, 1]^n : \sum_i x_i = \ell \}$.
% Then we can find an optimal solution $p^* \in \Delta_1$ to 
% $\argmax_{p \in\Delta_1} min_{c\in\Delta_{n-m}} f(p,c)$ in linear time, assuming we are given $g_i$ in sorted order, i.e. $g_1 \geq g_2 \geq g_3 \geq \ldots \geq g_n$.

% Define $H_k = \sum_{i \leq k} 1/g_i$, and
% let $N(k) = (k - m(1+w)) / H_k$. Then the solution is given by
% $$
% k^* = \argmax_{k\ge m(1+w)} N(k)
% $$
% and
% \begin{align*}
% p_i^* 
%     =&
%         \frac{1}{g_i H_{k^*}} \mbox{\ \ if $i \leq k^*$}
%         \mbox{\ \ and $p_i^*=0$ otherwise.}
% \end{align*}
% The maximum value $\min_{c\in\Delta_{n-m}} f(p^*, c)$ is $N(k^*)$.
% \end{lemma} 
% \begin{proof}
% Our proof relies on the the Minimax Theorem~\cite{neumann1928theorie}, which yields
% $$
% \min_{c\in\Delta_{n-m}} \max_{p\in\Delta_1} f(p,c) = \max_{p\in\Delta_1} \min_{c\in\Delta_{n-m}} f(p,c).
% $$

% Before beginning, we will first simplify $f(p,c)$ somewhat, finding
% \begin{align*}
% f(p, c) 
%     =& \sum_i g_i p_i c_i - \sum_i w g_i p_i (1-c_i)\\
%     =& \sum_i (c_i(1+w) - w) g_i p_i
% \end{align*}

% Now, consider the value $\min_{c\in\Delta_{n-m}} f(p^*, c)$, where $p^*$ is defined as in the lemma's statement. Notice that $g_i p_i^* = 1 / H_{k^*}$ for $i\leq k^*$, and 0 otherwise.
% Substituting, we see
% \begin{align*}
% f(p^*, c)
%     =& \sum_i (c_i(1+w) - w) g_i p^*_i \\
%     =& \sum_{i\leq k^*} (c_i(1+w) - w) / H_{k^*} \\
%     =& \frac{1+w}{ H_{k^*}} \sum_{i\leq k^*} c_i - k^*\frac{w}{ H_{k^*}}
% \end{align*}
% Clearly, this is minimized by making $c_i = 1$ for all $i>k^*$, leaving
% $\sum_{i\leq k^*} c_i = k^*-m$. Hence,
% \begin{align*}
% \min_{c\in\Delta_{n-m}} f(p^*, c)
%     =& \frac{1+w}{ H_{k^*}} (k^*-m) - k^*\frac{w}{ H_{k^*}} \\
%     =& \frac{k^*-m(1+w)}{ H_{k^*}} = N(k^*)
% \end{align*}
% This does not yet prove that $p^*$ is optimal, but it does show that
% $$
% N(k^*) = \min_{c\in\Delta_{n-m}} f(p^*, c)
%     \leq \max_{p\in\Delta_1} \min_{c\in\Delta_{n-m}} f(p, c)
% $$

% To show optimality, we'll provide a choice for $c$, denoted $c^*$, and show that $\max_{p\in\Delta_1} f(p, c^*) = N(k^*)$. Combined with the Minimax Theorem, this will be enough to complete the proof.

% To this end, define
% \begin{align*}
% c^*_i =& \begin{cases}
%     \frac{1}{1+w} \left( N(k^*)/g_i + w \right) \mbox{\ \ if $i\leq k^*$}    \\
%     1 \mbox{\ \ otherwise}
%     \end{cases}
% \end{align*}
% Notice that $\sum_i c^*_i = n - m$. Further,
% $c_i^*(1+w) - w = N(k^*)/g_i$ for $i\leq k^*$, and 1 otherwise.
% Substituting, we see
% \begin{align*}
% f(p, c^*)
%     =& \sum_i (c_i(1+w) - w) g_i p_i \\
%     =& \sum_{i\leq k^*} N(k^*) p_i + \sum_{i> k^*} g_i p_i 
% \end{align*}
% Before continuing, we observe that $N(k^*) \ge g_i$ for $i> k^*$. (To see this, we'll use the easy-to-prove rule that $\frac{a}{b} \geq \frac{a+c}{b+d}$ implies $\frac{a}{b} \geq \frac{c}{d}$ for positive numbers. The observation then follows since $N(k^*) \ge N(k^*+1)$, where $N(k^*) = \frac{k-m(1+w)}{H_{k^*}}$ and
% $N(k^*+1) = \frac{k-m(1+w) + 1}{H_{k^*} + 1/g_{k^*+1}}$.)

% So, $f(p, c^*)$ is maximized when $p_i = 0$ for $i > k^*$. Since $\sum_i p_i = 1$, we see $\max_{p\in\Delta_1} f(p, c^*) = N(k^*) \geq \min_{c\in\Delta_{n-m}} \max_{p\in\Delta_1} f(p, c)$. Applying Minimax and our earlier result, we have
% \begin{align*}
% N(k^*) = \min_{c\in\Delta_{n-m}} f(p^*, c)
%     \leq \max_{p\in\Delta_1} \min_{c\in\Delta_{n-m}} f(p, c)
%     = \min_{c\in\Delta_{n-m}} \max_{p\in\Delta_1} f(p, c)
%     \leq N(k^*)
% \end{align*}
% That is, $p^*$ attains the maximum value, as we wanted.
% \end{proof}


% \ignore{
% \subsection{Graveyard}

% \begin{align*}
% N(k^*) &\geq N(k^*+1) \\
% \frac{k-M}{H_{k^*}} &\geq \frac{k-M+1}{H_{k^*} + 1/g_{k^*+1}}\\
% (k-M)(H_{k^*} + 1/g_{k^*}) & \geq (k-M + 1) H_{k^*} \\
% (k-M)/g_{k^*} &\geq H_{k^*} \\
% N(k^*) &\geq g_{k^*}
% \end{align*}
% }  %% end ignore

==> Robust Active Distillation/sec/prefix.tex <==

\section{Proof for prefix with general penalties}

\begin{lemma}
\label{lem:minimax-max-gain}
Given $g_1 \geq g_2 \geq g_3 \geq \ldots \geq g_n > 0$ and $\ell_i \ge 0$ for $i\in\{1, 2, \ldots, n\}$, let
$f(p, c) = \sum_i g_i p_i (1-c_i) - \sum_i \ell_i p_i c_i$. Also let
$G_k = \sum_{i\leq k} \frac{g_i}{g_i+\ell_i}$ and 
$H_k = \sum_{i\leq k} \frac{1}{g_i+\ell_i}$.

Let $\gamma:\{1, 2, \ldots, n\} \rightarrow \mathbb{R}$ be an increasing function, and define
\begin{align*}
\Delta_{\gamma} = \{ x\in [0, 1]^n : \forall_k, \sum_{i\le k} x_i \leq \gamma(k) \}
\end{align*}
(We write $\Delta_1 = \{ x\in [0, 1]^n : \forall_k, \sum_{i\le k} x_i \leq 1 \} = \{ x\in [0, 1]^n : \sum_{i\le n} x_i \leq 1 \}$.)
Suppose $G_n \geq \gamma(n)$.
Then we can find an optimal solution $p^* \in \Delta_1$ to 
$\argmax_{p \in\Delta_1} min_{c\in\Delta_\gamma} f(p,c)$ in linear time.
 
The solution is given by
$$
k^* = \argmax_{k\ge m} \frac{G_k - \gamma(k)}{H_k}
$$
and
\begin{align*}
p_i^* 
    =&
        \frac{1}{H_{k^*}(g_i+\ell_i)} \mbox{\ \ if $i \leq k^*$}
        \mbox{\ \ and $p_i^*=0$ otherwise.}
\end{align*}
The maximum value $\min_{c\in\Delta_\gamma} f(p^*, c)$ is $N(k^*)$, where $N(k)$ is defined to be $\frac{G_k-\gamma(k)}{H_k}$.
\end{lemma} 
\begin{proof}
The proof relies on the the Minimax Theorem~\cite{neumann1928theorie}, which yields
$$
\min_{c\in\Delta_\gamma} \max_{p\in\Delta_1} f(p,c) = \max_{p\in\Delta_1} \min_{c\in\Delta_\gamma} f(p,c).
$$
We will further use two claims, which we'll prove shortly.

\begin{Claim}\label{claim:p}
Let $p^*$, $k^*$, and $N(k)$ be defined as in the statement of the lemma. Then $p^*\in\Delta_1$ and $N(k^*) = \min_{c\in\Delta_\gamma} f(p^*, c)$.
\end{Claim}

\begin{Claim}\label{claim:c}
Let $k^*$ and $N(k)$ be defined as in the statement of the lemma. Further, define
\begin{align*}
c^*_i =& 
    \max\left(0, \frac{g_i - N(k^*)}{g_i + \ell_i}\right)
\end{align*}
Then $c^*\in\Delta_\gamma$ and
$N(k^*) = \max_{p\in\Delta_1} f(p, c^*)$.
\end{Claim}
Given the claims, we see
\begin{align*}
N(k^*) = \min_{c\in\Delta_\gamma} f(p^*, c) 
    \leq& \max_{p\in\Delta_1} \min_{c\in\Delta_\gamma} f(p, c) \mbox{\ \ by Claim~\ref{claim:p}} \\
    =& \min_{c\in\Delta_\gamma}\max_{p\in\Delta_1} f(p, c) \mbox{\ \ by Minimax} \\
    \leq& \max_{p\in\Delta_1} f(p, c^*) = N(k^*) \mbox{\ \ by Claim~\ref{claim:c}}
\end{align*}
That is, $p^*$ attains the maximum, which is $N(k^*)$, as we wanted.

We now prove the claims.
Before beginning, we will first simplify $f(p,c)$ somewhat, finding
\begin{align*}
f(p, c) 
    =& \sum_i g_i p_i(1- c_i) - \sum_i \ell_i p_i c_i\\
    =& \sum_i (g_i - c_i(g_i + \ell_i)) p_i
\end{align*}
\begin{proof}[Proof of Claim~\ref{claim:p}]
We first show $p^*\in\Delta_1$. We have
\begin{align*}
\sum_{i\leq n} p^*_i = \sum_{i\leq k^*} p^*_i 
    = \sum_{i\leq k^*} \frac{1}{H_{k^*}(g_i+\ell_i)} 
    = \frac{H_{k^*}}{H_{k^*}} = 1
\end{align*}
And since $p^*_i \ge 0$ for all $i$, it immediately follows that $p^*_i \leq 1$ as well.

We now show $N(k^*) = \min_{c\in\Delta_{n-m}} f(p^*, c)$. To this end,
\begin{align*}
f(p^*, c)
    =& \sum_{i\leq n} (g_i - c_i(g_i + \ell_i)) p_i \\
    =& \sum_{i\leq k^*} \frac{g_i - c_i(g_i + \ell_i)}{H_{k^*}(g_i+\ell_i)} \\
    =& \sum_{i\leq k^*} \frac{g_i}{H_{k^*}(g_i+\ell_i)} -
    \sum_{i\leq k^*} \frac{c_i} {H_{k^*}} \\
    =&  \frac{G_{k^*}}{H_{k^*}} -
   \frac{1} {H_{k^*}}  \sum_{i\leq k^*} c^*_i
\end{align*}
Clearly, for $c^*\in\Delta_\gamma$, this expression is minimized when $\sum_{i\leq k^*} c_i = \gamma(k^*)$.
\enote{We need a little more here. Basically, we want to set $c_i = 1$ for $i\in [k^*-\gamma(k^*)+1, k^*]$ and $c_i =0$ otherwise. So long $\gamma$ allows this, we're happy. Otherwise, things get weird.}
So we have
\begin{align*}
\min_{c\in\Delta_\gamma} f(p^*, c)
    &= \frac{G_{k^*}}{H_{k^*}} -\frac{\gamma(k^*)} {H_{k^*}}
    = N(k^*)
\end{align*}
as claimed.
\end{proof}

We now prove our second claim.
\begin{proof}[Proof of Claim~\ref{claim:c}]
We first show that $N(k^*) \ge g_i$ for $i>k^*$.\footnote{In the border case that $k^*=n$, we can add a dummy item with $g_{n+1}=0$ and the claim follows trivially.}
Observe that if $\frac{a}{b} \ge \frac{a+c}{b+d}$, then $\frac{a}{b} \ge \frac{c}{d}$ for non-negative values (and $b>0, d>0$).
Notice
\begin{align*}
\frac{G_{k^*}-m}{H_{k^*}} = N(k^*)\ge  
N(k^*+1) =\frac{G_{k^*}+g_{k^*+1}/(g_{k^*+1}+\ell_{k^*+1})-m}{H_{k^*}+1/(g_{k^*+1}+\ell_{k^*+1})} 
\end{align*}
By our observation,
$$
N(k^*) \ge \frac{g_{k^*+1}/(g_{k^*+1}+\ell_{k^*+1})}{1/(g_{k^*+1}+\ell_{k^*+1})} = g_{k^*+1} \ge g_i \mbox{\ \ for $i>k^*$.}
$$
Similarly, we show $N(k^*) \le g_i$ for $i\leq k^*$, using the observation that if $\frac{a-c}{b-d} \leq \frac{a}{b}$, then $\frac{a}{b} \le \frac{c}{d}$ for non-negative values (and $b-d>0$ and $d>0$).
Notice
\begin{align*}
N(k^*-1) = 
\frac{G_{k^*}-g_{k^*}/(g_{k^*}+\ell_{k^*})-m}{H_{k^*}-1/(g_{k^*}+\ell_{k^*})} 
\leq \frac{G_{k^*}-m}{H_{k^*}}
= N(k^*)
\end{align*}
And again, by our observation,
$$
N(k^*) \le \frac{g_{k^*}/(g_{k^*}+\ell_{k^*})}{1/(g_{k^*}+\ell_{k^*})} = g_{k^*} \le g_i \mbox{\ \ for $i\le k^*$.}
$$
Now we're ready to prove the claim.

We first show $c^*\in\Delta_{n-m}$. Since $N(k^*) \le g_i$ for $i\le k^*$, we see
$c^*_i = \frac{N(k^*)+\ell_i}{g_i + \ell_i} \le 1$ for $i\le k^*$. So $c^*_i \in [0, 1]$. Further,
\begin{align*}
\sum_{i\le n} c^*_i
    =& \sum_{i\le k^*} \frac{N(k^*)+\ell_i}{g_i + \ell_i} + \sum_{k^* < i \le n} 1 \\
    =& \sum_{i\le k^*} \frac{N(k^*)-g_i}{g_i + \ell_i} + \sum_{i\le k^*}\frac{g_i+\ell_i}{g_i + \ell_i}  +\sum_{k^* < i \le n} 1 \\
    =& N(k^*) H_{k^*} - G_{k^*} + n \\
    =& G_{k^*} - m - G_{k^*} + n = n-m
\end{align*}
That is, $c^*\in\Delta_{n-m}$.

Finally, we show $N(k^*) = \max_{p\in\Delta_1} f(p, c^*)$. Note that 
$c^*_i(g_i+\ell_i) - \ell_i = N(k^*)$
for $i\le k^*$, while 
$c^*_i(g_i+\ell_i) - \ell_i = g_i$ for $i> k^*$.
We have
\begin{align*}
f(p, c^*) 
    =& \sum_i (c^*_i(g_i + \ell_i) - \ell_i) p_i\\
    =& \sum_{i\leq k^*} N(k^*) p_i
        +\sum_{i> k^*} g_i p_i
\end{align*}
From above, $N(k^*) \ge g_i$ for $i>k^*$. So the expression is maximized for $p\in\Delta_1$ when $p_i = 0$ for $i> k^*$ and $\sum_{i\leq k^*} p_i = 1$. Hence,
\begin{align*}
\max_{p\in\Delta_1} f(p, c^*) = N(k^*)
\end{align*}
as we wanted.
\end{proof} %% End proof of claim.
\end{proof} %% End proof of lemma.


\ignore{
\subsection{Graveyard}

\begin{align*}
N(k^*) &\geq N(k^*+1) \\
\frac{k-M}{H_{k^*}} &\geq \frac{k-M+1}{H_{k^*} + 1/g_{k^*+1}}\\
(k-M)(H_{k^*} + 1/g_{k^*}) & \geq (k-M + 1) H_{k^*} \\
(k-M)/g_{k^*} &\geq H_{k^*} \\
N(k^*) &\geq g_{k^*}
\end{align*}
}  %% end ignore

==> Robust Active Distillation/sec/problem-statement.tex <==
\section{Problem Statement}
\label{sec:problem-statement}

We consider the semi-supervised classification setting where we are given a small labeled set \rev{$\XX_L$ -- typically tens or hundreds of thousands of examples -- together with a large unlabeled set $\XX_U$}, typically on the order of millions or billions. The goal is to leverage both the labeled and unlabeled sets to efficiently and reliably train a compact, powerful model $\student$. \reviclr{To do so, we use knowledge distillation~\cite{xie2020self,liang2020mixkd} where the labeled points are used to train a larger, (often pre-trained) teacher model that can then be used to educate a small model (the \emph{student})}. \reviclr{We emphasize that the teacher may be a pre-trained model, however, it is not trained on the unlabeled set $\XX_U$. The distillation process entails using the soft-labels of the teacher for the unlabeled points. The student is then trained on these soft-labeled points along with the original labeled data set.}
\reviclr{The key insight is that the large, pre-trained teacher model can more aptly learn representations from the limited  data, which can then be imitated by the student.}

\rev{
Somewhat more formally, we are given two input sets $\XX_L, \XX_U$ independently and randomly drawn from the input space $\XX \subseteq \Reals^d$. We assume that we have access to the hard labels $\YY_L \in \{0, 1\}^k$ for the instances in $\XX_L$, but not those in $\XX_U$ and that $|\XX_L| \ll |\XX_U|$.  \reviclr{Consistent with modern ML applications, we assume that a validation data set of labeled points is available.}
%, e.g., $|\XX_A|$ may be a couple thousand and $|\XX_B|$ on the order of millions or billions. 
% , however, that a very limited number of groundtruth label queries can be made for the points in $\XX_U$ throughout the distillation process. 
We will use a slight abuse in notation and refer to the set of labeled data points as $(\XX_L, \YY_L)$ to denote the set of $(x,y)$ labeled pairs. We assume large-scale applications of KD where the teacher is exceedingly large to the extent that querying the teacher soft-label $f_{\teacher}(x) \in [0,1]^k$ for an unlabeled point $x \in \XX_U$ is costly and soft-labeling all of $\XX_U$ is infeasible. In the following, we introduce and motivate robust active distillation to conduct this process efficiently and reliably.}


%% Original...
\ignore{
We consider the semi-supervised classification setting where we are given two input sets $\XX_A, \XX_B$ independently and randomly drawn from the input space $\XX \subseteq \Reals^d$. We assume that we have access to the hard labels $\YY_A \in \{0, 1\}^k$ for the instances in $\XX_A$, but not those in $\XX_B$ and that $|\XX_A| \ll |\XX_B|$, e.g., $|\XX_A|$ may be a couple thousand and $|\XX_B|$ on the order of millions or billions. 
\enote{Do we still need this assumption if we don't do the bucket approach?} \knote{I think this is a fair assumption. Basically, it says that we don't have many labeled examples? The next assumption that it's expensive getting soft labels from the teacher is even stronger.} \cnote{I had put this to describe the problem setting where our method could be of most help, since if $|\XX_A| \approx |\XX_B|$ then we could just soft-label entirety of $\XX_B$} 
We do assume, however, that a very limited number of groundtruth label queries can be made for the points in $\XX_B$ throughout the distillation process. We will use a slight abuse in notation and refer to the set of labeled data points as $(\XX_A, \YY_A)$ to denote the set of $(x,y)$ labeled pairs, and for a given subset $\SS \subseteq \XX_B$ with teacher soft labels $\tilde \YY_{\SS}$ we will let $(\SS, \tilde \YY_{\SS})$ denote the set of soft-labeled pairs. We assume large-scale applications of KD where the teacher is exceedingly large to the extent that querying the teacher soft-label $f_{\teacher}(x) \in [0,1]^k$ for an unlabeled point $x \in \XX_B$ is highly expensive computationally and soft-labeling all of the points in $\XX_B$ is infeasible.

\enote{Maybe a little more description of our set-up in words?} \cnote{I added the following, happy to elaborate further}\enote{Looks good. Originally, I thought this description should be the first para. I'm not sure right now.} \cnote{Good point. I'm torn between which one should come first. Any suggestions?}
At a high level, our goal is to leverage both the labeled and unlabeled sets to efficiently and reliably train a compact, powerful model $\student$. To do so, we use knowledge distillation and follow the setup of prior work~\cite{xie2020self,liang2020mixkd} where the labeled points are used to train a larger model (the \emph{teacher}) that can then be used to educate a light-weight model (the \emph{student}). Following the standard paradigm~\cite{hinton2015distilling}, this entails using the soft-labels (i.e., normalized categorical prediction) of the teacher for the points that are unlabeled. The student is then trained on these soft-labeled points along with the original labeled data set. The key insight is that the large teacher model can more aptly learn representations from the limited labeled data, which can then be imitated by the student. In the following, we introduce and motivate robust active distillation to conduct this process efficiently and reliably.
} %% end ignore
%In this paper, we assume that we have access to a high-capacity teacher model $\teacher$ trained on the set of labeled pairs $(\XX_A, \YY_A)$. We specifically consider the scenario where We formalize this goal in the following and underscore the shortcomings of existing approaches.
%teacher soft labels for only a small, judiciously chosen subset of points in $\XX_B$ 

\subsection{Active Distillation}

%In knowledge distillation, we first train a high-capacity teacher model $\teacher$ on the small set of labeled data $(\XX_A, \YY_A)$.  
\reviclr{The objective of active distillation is to query the minimum number of teacher soft-labels for points in $\XX_U$ in order to train a high-performing student model $\theta_\mathrm{student}$ in a computationally and financially-efficient way}. This process is shown in  Alg.~\ref{alg:active-distillation}. Here, we conduct $T$ active distillation iterations after training the student and the teacher models on the training set $\PP$, which initially only includes the set of hard-labeled points.  On Line~\ref{lin:soft-label} and throughout, $f_\theta(x) \in [0,1]^k$ denotes the softmax output of a neural network model $\theta$ with respect to input $x$. At each iteration (Lines~\ref{lin:start-active}-\ref{lin:end-active}, Alg.~\ref{alg:active-distillation}), we use a given querying algorithm, \textsc{Select}, to identify the most helpful $b$ unlabeled points to soft-label by the teacher based on the most up-to-date student model $\theta_{t-1}$ (Line~\ref{lin:select}). The selected points are then soft-labeled by the teacher and added to the (expanding) training set $\PP$. Subsequently, the student is trained using the Kullback-Leibler (KL) Divergence~\cite{hinton2015distilling} as the loss function on the training set $\PP$ which includes both the hard-labeled points $(\XX_L, \YY_L)$ and the accumulated soft-labeled ones. We follow the standard convention in active learning~\cite{ren2021survey} and efficient distillation ~\cite{liang2020mixkd,xu2020computation} and train the student model from scratch on Line~\ref{lin:train}.

\input{sec/method}

% We train the lightweight student model on the union of the set of labeled points $(\XX_A, \YY_A)$ and the set of soft-labeled points $(\SS, \cup_{x \in \SS} f_{\student}(x))$. For the soft-labeled points, we follow the paradigm of~\cite{hinton2015distilling} and use the Kullback-Leibler (KL) Divergence for the loss when training the student on unlabeled data points,
% $$
% \mathrm{KL}(f_{\teacher}(x), f_{\student}(x)) = \sum_{i \in [k]} f_{\teacher}(x)_i \log(f_{\teacher}(x)_i / f_{\student}(x)_i),
% $$
% where $f_{\student}(x) \in [0,1]^k$ is the softmax output of the student, and cross-entropy loss with respect to the true label for the labeled points. 


The active distillation problem is deeply related to the problem of \emph{active learning}, where the objective is to query the labels of only the most informative points in order to minimize labeling costs. To this end, prior approaches in efficient KD~\cite{xu2020computation,liang2020mixkd} have proposed methods inspired by margin-based sampling~\cite{balcan2007margin,roth2006margin}, a popular and widely used active learning algorithm~\cite{ren2021survey}. Margin-based sampling is one example of uncertainty-based sampling, other examples are clustering-based selection~\cite{sener2017active,ash2019deep}, model uncertainty~\cite{gal2017deep}, and adversarial proximity~\cite{ducoffe2018adversarial} (see~\cite{ren2021survey} for a survey). In the following, we consider margin-based sampling due to its simplicity and prior application to efficient distillation by related work~\cite{liang2020mixkd,xu2020computation}. Margin-based sampling for KD is an intuitive and simple-to-implement idea where the teacher predictions for inputs that the student is most uncertain about are queried. For an input $x$ and prediction $i^* = \argmax_{i \in [k]} f_{\student}(x)_i$, the uncertainty is measured in terms of the \emph{margin} between the top-2 highest probability entries, i.e.,
$
\mathrm{margin}(x) = f_{\student}(x)_{i^*} - \max_{i \in [k] \setminus i^*} f_{\student}(x)_i.
$

\begin{figure*}[ht!]
  \centering
  \begin{minipage}[t]{0.52\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/misc/margin_plot_v2.png}
  \end{minipage}%
  \centering
  \begin{minipage}[t]{0.48\textwidth}
  \centering
   \includegraphics[width=1\textwidth]{figs/misc/with-cheating}
  \end{minipage}%
\caption{\textbf{Left:} \rev{teacher's accuracy (overall $60.7\%$) relative to the student's (overall $49.4\%$) \emph{margin score}; points with lower margin tend to be incorrectly classified by the teacher. Plot was generated by  averaging teacher's accuracy over 100 closest-margin points.} \textbf{Right:} Performance of robust distillation (red), which picks the lowest-margin points \emph{among those correctly labeled by the teacher}, compared to that of margin (blue).}
%Points with lower student margin scores tend to be incorrectly labeled by the teacher.}
%We use a k-NN to compute the probability that the teacher is correct for a given margin.
\label{fig:margin}
\end{figure*}

\subsection{\rev{Research Gap}}


Despite the widespread success of margin-based sampling in active learning, we claim that it is generally ill-suited for knowledge distillation due to its tendency to amplify confirmation bias, leading to poor student performance. To observe this, note that the objective of margin-based sampling -- and more generally, other uncertainty-based query methods -- is to query the soft-labels of inputs for which the student is most uncertain about ("hard" instances). However, hard instances for the student are often hard to predict correctly by the teacher. Hence, the soft-labels for these points are more likely to be incorrect with respect to the groundtruth labels, leading to misleading student training. 




Fig.~\ref{fig:margin} shows an instance of this phenomenon for CIFAR10 with ResNet student-teacher architectures of varying depth. As the figure depicts, the teacher tends to predict incorrect labels for points with low student margin (hard instances), and conversely, tends to be highly accurate on points with high margin (easy instances). This suggests that there is an inherent trade-off between efficiency (minimizing queries) and robustness (mitigating confirmation bias) that needs to be considered. That is, we would like to pick informative points for the student for efficiency, but these informative points tend to be incorrectly classified by the student which leads to misguided training and poor performance. Is it possible to simultaneously achieve both in a principled way? We label this problem \emph{Robust Active Distillation} and propose a method to solve it in the following section.



==> Robust Active Distillation/sec/proof_sketch.tex <==

\newcommand{\obj}{\textsc{Obj}}
\newcommand{\opt}{\textsc{OPT}}
\newcommand{\defeq}{\mathrel{\mathop:}=}

%\begin{theorem}

%\begin{restatable*}{thm}
\begin{restatable*}{thm}{minimaxmaxgain}
\label{thm:minimax-max-gain}
Suppose $g_1 \geq g_2 \geq \cdots \geq g_n > 0$, and define $G_k = \sum_{i\leq k} g_i / (g_i+\ell_i)$ and
$H_k = \sum_{i\leq k} 1 / (g_i+\ell_i)$.
For $G_n\ge m$,
an optimal solution $p^*\in\Delta_1$ to \eqref{prb:ours-general} is given by
\begin{align*}
p_i^* 
    =& \frac{1}{H_{k^*}(g_i+\ell_i)} \mbox{\ \ if $i \leq k^*$}
        \mbox{\ \ and $p_i^*=0$ otherwise, where \ }
        k^* = \argmax \nolimits_{k\in[n]} \frac{G_k - m}{H_k}.
\end{align*}
The distribution can be computed in linear time (assuming sorted $g$) and achieves an objective value of
$\opt(k^*) \defeq \frac{G_{k^*} - m}{H_{k^*}}$.
%\end{theorem} 
\end{restatable*}
We sketch the proof here. The full proof can be found in the Appendix (Sec.~\ref{sec:supp-analysis}).
\begin{proof}[Proof sketch]
Let $$\obj(p,c) = \sum_{i \in [n]} p_i (g_i c_i - (1-c_i)\ell_i).$$
Substituting $p^*$ from Thm.~\ref{thm:minimax-max-gain} and considering a minimizing value for $c\in\Delta_{n-m}$, it is possible to show that 
$p^*\in\Delta_1$ and
$$
\opt(k^*) 
%= \frac{G_{k^*} - m}{H_{k^*}}  
= \min_{c\in\Delta_{n-m}} \obj(p^*, c) \leq \max_{p\in\Delta_1} \min_{c\in\Delta_{n-m}} \obj(p, c).
$$
On the other hand, let $c_i^* = \min \big(1, \frac{\opt(k^*) + \ell_i}{g_i+\ell_i}\big)$. With a little more work, using the fact that
$g_{k^*} \ge \opt(k^*) \ge g_{k^*+1}$,
we can show similarly that $c^*\in\Delta_{n-m}$ and
$$
\opt(k^*) = \max_{p\in\Delta_{1}} \obj(p, c^*) \geq \min_{c\in\Delta_{n-m}} \max_{p\in\Delta_1} \obj(p, c).$$
With these inequalities in hand, we apply the Minimax Theorem~\cite{neumann1928theorie}, which yields
$$
\opt(k^*) \leq 
\max_{p\in\Delta_1} \min_{c\in\Delta_{n-m}} \obj(p, c)
= \min_{c\in\Delta_{n-m}} \max_{p\in\Delta_1} \obj(p, c)
\leq \opt(k^*).
$$
Hence, $p^*$ does indeed obtain the optimal value, $\opt(k^*)$.
\end{proof}

\ignore{
\enote{I think I prefer the above proof sketch. It's shorter and nicer to look at. I don't think the extra details make us look any smarter.}
\begin{proof}[Proof sketch with a few more details]
Let $\obj(p,c) = \sum_i p_i (g_i c_i - (1-c_i)\ell_i)$. Substituting $p^*$ and rearranging, it is possible to show that $\obj(p^*, c) = \frac{1}{H_{k^*}}\sum_{i\le k^*} (c_i + G_{k^*} - k^*)$. The minimum is attained when $\sum_{i\leq k^*} c_i = k^* - m$, yielding the value $\frac{G_{k^*} - m}{H_{k^*}} = \opt(k^*)$. Since $p^*\in\Delta_1$, we have
$$
\opt(k^*) 
%= \frac{G_{k^*} - m}{H_{k^*}}  
= \min_{c\in\Delta_{n-m}} \obj(p^*, c) \leq \max_{p\in\Delta_1} \min_{c\in\Delta_{n-m}} \obj(p, c).
$$
On the other hand, let $c^* = \min \left(1, \frac{\opt(k^*) + \ell_i}{g_i+\ell_i}\right)$. With a little work, we can show the wonderful fact that
$g_{k^*} \ge \opt(k^*) \ge g_{k^*+1}$, which in turn gives us
$c^*\in\Delta_{n-m}$. Substituting and rearranging, we can arrive at $\obj(p, c^*) = \sum_{i\leq k^*} \opt(k^*) p_i + \sum_{i>k} g_i p_i$. Since (by our wonderful fact) $\opt(k^*) \ge g_{k^*+1}$, this quantity is maximized when $p_1 = 1$, yielding
$$
\opt(k^*) = \max_{p\in\Delta_{1}} \obj(p, c^*) \geq \min_{c\in\Delta_{n-m}} \max_{p\in\Delta_1} \obj(p, c).
$$
Finally, we apply the Minimax Theorem, which shows
$$
\opt(k^*) \leq 
\max_{p\in\Delta_1} \min_{c\in\Delta_{n-m}} \obj(p, c)
= \min_{c\in\Delta_{n-m}} \max_{p\in\Delta_1} \obj(p, c)
\leq \opt(k^*)
$$
Hence, $p^*$ does indeed obtain the maximum value, $\opt(k^*)$.
\end{proof}
}

==> Robust Active Distillation/sec/rad-old-good-state.tex <==
\section{Robust Active Distillation (RAD)}
\label{sec:rad}
In this section, we motivate and present our approach, $\mathrm{RAD}$, that explicitly considers the competing objectives of efficiency and robustness in knowledge distillation.

\subsection{Problem Statement}

Recall that the margin algorithm~\cite{liang2020mixkd,roth2006margin} selects the $b$ points with the lowest margin scores $\mathrm{margin}(x)$, where $b$ is our soft-label budget. Let $\margin$ be shorthand for the margin of each unlabeled input $\mathrm{margin}(x_i)$ and observe that its \emph{gain} or informativeness can be quantified as
$$
\gain = (1 - \margin).
$$
Given a budget $b$, note that the margin-sampling algorithm corresponds to the optimal solution of the following optimization problem where the objective is to generate a probability distribution that maximizes the sum of gains,
\begin{equation}
\label{eqn:naive-max-gain}
\max_{p \in \Delta_b} \E_{\SS \sim p} \Big[\sum_{i \in \SS} g_i\Big] \, \,  \text{, where } \Delta_b = \{p \in [0,1]^n: \sum_{i \in [n]} p_i = b\}.
\end{equation}
As discussed previously. this formulation solely focused on the informativeness of the points and does not consider the increased likelihood of mislabeling by the teacher.



\paragraph{Robust Distillation} To extend  \eqref{eqn:naive-max-gain} so that it considers robustness, consider the masks
$$
c_i = \1 \{\text{teacher labels point i correctly}\} \quad \forall{i \in [n]},
$$
where $\1 \{x \} = 1$ if $x$ is true and 0 otherwise. Equipped with this additional variable, one way to
explicitly mitigate confirmation bias and simultaneously pick informative samples is to reward points that are correctly labeled by the teacher by assigning gains as before, but penalize those that are incorrectly labeled via losses. This can be done by using the modified gains in the context of \eqref{eqn:naive-max-gain}
$$
\tilde g_i = g_i c_i - (1 - c_i) \ell_i = \begin{cases}
g_i, &\text{ if teacher labels point i correctly} \\
-\ell_i, &\text{ otherwise }
\end{cases} \quad \forall{i \in [n]}.
$$
In words, this means that if the point $i$ is correctly labeled by the teacher we assign the standard margin-based gain $g_i = (1 - \margin)$ as before; otherwise, we penalize the selection by assigning $-\ell_i$ for some loss $\ell_i \ge 0$. This leads to the following general problem of robust distillation
\begin{equation}
    \label{prb:general}
    \max_{p \in \Delta_1} \E \nolimits_{i \sim p} \left[g_i c_i - (1 - c_i) \ell_i \right].
\end{equation}


\paragraph{Zero-loss Setting} For sake of simplicity, we assume henceforth that we are sampling a single point, i.e., $b = 1$. Setting the losses $\ell_i = 0$ for all $i \in [n]$ leads to the following modification of \eqref{eqn:naive-max-gain}
\begin{equation}
\label{eqn:max-gain-zero-loss}
\max_{p \in \Delta_1} \E \nolimits_{i \sim p} \left[g_i c_i \right],
\end{equation}
which encourages the selection of points that are correctly labeled since picking an incorrect point does not contribute at all towards the gain. The formulation in \eqref{eqn:max-gain-zero-loss} encourages selecting instances that have high gains and are labeled correctly by the teacher, however, it does not at all account for the \emph{damage} that incorrectly labeled ones can have on the student. Prior work on confirmation bias has shown that even a small number misguided soft-labels can derail the student's performance and significantly impact its predictive capability~\cite{liu2021certainty}. Additionally, the harm of an incorrectly labeled point may be even more pronounced when the student is uncertain about that point. 
%(i.e., high gain) about the data point to begin with. 

\paragraph{Relative Loss} To overcome the limitations of the previous formulation, we consider instantiating the general framework \eqref{prb:general} with losses that are \emph{relative to the gain} $\ell_i = -w g_i$ for each $i \in [n]$ where $w \in [0,1]$ is a weight parameter that controls the magnitude of the penalization. This relative formulation purposefully leads to higher penalties misclassified points that the student is already unsure about (high gain) to mitigate confirmation bias, and leads to the following optimization problem which we consider in this paper
\begin{equation}
\label{prb:relative-ground-truth-prob}
\max_{p \in \Delta_1} \E \nolimits_{i \sim p} \left[g_i c_i - (1 - c_i) w g_i \right].
\end{equation}

The optimal solution to problem  \eqref{prb:relative-ground-truth-prob} corresponds to picking the most informative (highest gain) points \emph{among those that are predicted correctly by the teacher}, i.e., those points $i \in [n]$ with highest $g_i$ subject to $c_i = 1$. This approach is shown as  Robust Distillation (Oracle) in Fig.~\ref{fig:margin} (right). As Fig.~\ref{fig:margin} and our additional results in Sec.~\ref{sec:supp-results} of the Appendix consistently show, if we have knowledge of $(c_i)_{i \in [n]}$, then we can optimally solve \eqref{prb:relative-ground-truth-prob} above to obtain significant improvements over the standard margin algorithm. Unfortunately, however, perfect knowledge of whether the teacher labels a point correctly or not, i.e., $(c_i)_{i\in[n]}$, is never possible in the semi-supervised learning setting.


% \enote{I'm not sure yet, but consider moving this discussion elsewhere.} \cnote{I agree. I'm open to suggestions on where to place it} \cnote{Update: should this just be removed?}
% Given the success of the formulation with the indicator-modified gains, one lingering question is whether we can apply the same approach when we do not have access to the indicators $(c_i)_{i \in [n]}$. One approach is to use predict the masks using an algorithm like k-Nearest Neighbor (k-NN) with the gains as the input space. Here the k-NN can be constructed using a validation set of points with both the groundtruth label and the teacher's softmax label for each point and used to infer the indicators $(c_i)_{i \in [n]}$. However, as seen in Fig.~\ref{fig:margin}, even though the general trend is that low margin (high gain) points $i$are misclassified more often, it is very difficult to predict the indicator $c_i$ for each point $i$ \emph{individually}. In Sec.~\ref{sec:} of the appendix, we additionally describe our attempts at using k-NNs with various input spaces, ranging from the student's embedding layer to the input itself, to no avail.

\subsection{Our Approach}

%\enote{Again, I'm not sure. This description saves space, and might be easier to understand for readers. Breaking it into (1) no penalty, then (2) penalty proportional to $wg_i$ tells a better story.} 
%\cnote{Done. Please let me know if this is the structure you had in mind.}
%% \enote{looks good. commenting out the notes}
We consider a general and robust approach that simultaneously leverages instance-specific knowledge without having to know the masks $(c_i)_{i\in [n]}$ individually. Suppose that we only knew that the teacher mislabels $m$ points out of the $n$ unlabeled inputs $\XX_B$. Can we generate a sampling distribution so that no matter which of the $m$ points are labeled incorrectly by the teacher, our expected gain is high? Assuming for simplicity that $b = 1$, this question leads to the following which extends \eqref{prb:relative-ground-truth-prob}
\begin{equation}
\label{prb:ours}
\max_{p \in \Delta_1} 
%\min_{c \in \{0, 1\}^n: \dotp{c}{\mathbf{1}} = n - m} 
\min_{c\in\Delta_{n-m}}
\E \nolimits_{i \sim p} \left[g_i c_i - (1 - c_i) w g_i \right],
\end{equation}
where $\Delta_k = \{q \in [0,1]^n: \sum_{i \in [n]} q_i = k\}$ as before. 

Problem~\eqref{prb:ours} has the following game theoretic interpretation. We go first and pick a sampling distribution $p$ over the points $n$. In response, an adversary decides which points are misclassified by the teacher subject to the constraint that it can set $c_i = 0$ for (i.e., misclassify) at most $m \leq n$ of them since $c \in \Delta_{n-m}$. By von Neumann's Minimax Theorem~\cite{neumann1928theorie} the objective value is the same regardless of whether we go first and pick the probability distribution or the adversary goes first and picks $(c_i)_{i \in [n]}$. In fact, it turns out that this observation applies to the analogue of the more general framework formulation~\eqref{prb:general} with arbitrary gains and losses, and this connection leads to a closed form solution for the optimal distribution as formalized in the theorem below.


\begin{figure*}[ht!]
  \centering
  \begin{minipage}[t]{0.49\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/misc/teacher-gain.png}
  \end{minipage}%
  \hfill
  %\hspace{3px}
  \begin{minipage}[t]{0.49\textwidth}
  \centering
   \includegraphics[width=1\textwidth]{figs/misc/teacher-point-idx.png}
  \end{minipage}%

\caption{The optimal solution to \eqref{prb:ours} given by Lemma~\ref{lem:single-sample-lemma} for various values for teacher accuracy (varying $m$). Even when most of the samples are labeled correctly by the teacher, our method is purposefully cautious and does not allocate all of the probability (of sampling) mass on the highest gain points.}
\label{fig:sampling-distribution}
\end{figure*}

\input{sec/proof_sketch}

\ignore{
\begin{lemma}
\label{lem:single-sample-lemma}
An optimal solution $p^* \in \Delta_1$ to \eqref{prb:ours} has $k$ non-zero entries $\II_{k^*} \subseteq [n]$ corresponding to the $k^*$ indices of the largest entries of $g$, with
$$
p^*_i = \frac{1}{g_i \sum_{j \in \II_{k^*}} g_j^{-1}} \quad \forall{i \in \II_{k^*}} \quad \text{where} \quad k^* = \argmax_{k \in [n]} \frac{k - (1 + w)m}{ \sum_{j \in \II_k} g_j^{-1}}.
$$
The distribution $p^*$ can be computed in $\Theta(n \log n)$ time and achieves an objective value of
$$\frac{k^* - (1 + w)m}{ \sum_{j \in \II_{k^*}} g_j^{-1}}.$$
\end{lemma} 
\begin{proof}
\enote{proof sketch} \cnote{Should the proof sketch be for the more general lemma in the appendix? But in that case maybe that doesn't belong in the proof of this lemma, since we are just applying Lemma~\ref{lem:minimax-max-gain} with $\ell_i = w g_i$ here}
Let $G(p, c) = \E \nolimits_{i \sim p} \left[g_i c_i - (1 - c_i) w g_i \right]$. By linearity of $G(p, c)$ and integrality of $n - m$ the minimum over the masks $c$ is attained at the boundary points, i.e.,
$$
\min_{c \in \{0, 1\}^n: \dotp{c}{\mathbf{1}}  = n - m} G(p, c) = \min_{c \in \Delta_{n-m}} G(p, c) \quad \forall{p \in \Delta_1}.
$$
This form now allows us to invoke von Neumann's Minimax Theorem~\cite{neumann1928theorie} to show that the optimal solution $p^*$ given above attains the optimal objective value. This is formalized in Lemma~\ref{lem:minimax-max-gain} of the Appendix and its application leads to the lemma statement.
\end{proof}
}


Fig.~\ref{fig:sampling-distribution} depicts examples of the optimal solution on a synthetic scenario with gains drawn uniformly at random from $[0,1]$. We observe that, contrary to the standard margin, our sampling distribution tends to allocate less probability mass to the highest gain items. On the other hand, like standard margin, it completely avoids sampling (i.e., assigns $0$ probability to) a large portion of low-gain points based on a certain threshold that is a function of the teacher's accuracy (reliability). Notably, the optimal solution to \eqref{prb:ours} is also reminiscent of a popular active learning heuristic, where the top-$2b$ points with highest gain are selected and among them $b$ points are sampled uniformly at random. In this regard, our formulation and analysis leads to its theoretical justification as a byproduct~\cite{citovsky2021batch}.


\subsection{Implementation Details}
We conclude this section by outlining the practical details of \textsc{Rad}. In particular, we detail the procedure used to sample a batch of points, approximate the value of $m$, and set the weight parameter $w$ in the context of \eqref{prb:ours}. In practice, we use the distribution $q = \min\{b p, 1\}$ when sampling a set of $b$ points, where $p$ is from Lemma~\ref{lem:single-sample-lemma}. This is optimal as long as the probabilities from Lemma~\ref{lem:single-sample-lemma} are not heavily concentrated on a few points (i.e., $\max_{i \in [n]} p_i \leq 1/b$). As exemplified in Fig.~\ref{fig:sampling-distribution} and experimentally verified in Sec.~\ref{sec:results} in all of the evaluated scenarios, we found this to always be the case. Alternatively, the acquisition size $b$ can be adjusted after the single-sample probability distribution is computed so that $b \leq \min_{i \in [n]} 1 / p_i$.
 
 Since the number of mistakes the teacher makes on $\XX_B$, $m$, is not known to us in the semi-supervised setting, we approximate this quantity by first taking the sample mean inaccuracy of a small uniform random sample of $b_\mathrm{uniform}$ points as a way to approximate $m$ and bootstrap our approach. We then use our approach with $b' = b - b_\mathrm{uniform}$ (i.e., $q = \min\{b' p, 1\}$) as described above. By Bernstein's inequality~\cite{bernstein1924modification}, this weighted estimate tightly concentrates around the mean, which in turn implies a high-quality approximation of $m$. The details of this procedure and the effect of using an approximate value of $m$ on the quality of the optimal solution to \eqref{prb:ours} are discussed in Sec.~\ref{sec:supp-analysis} of the Appendix. Finally, we use the weight $w = (1 - m/n)$ as the relative penalization constant. This choice of $w$ ensures that the optimal value of~\ref{prb:ours} as specified by Lemma~\ref{lem:single-sample-lemma} is non-negative (and in fact, proportional to $(n - m)^2/n$), which justifies the sampling procedure in the first place.\footnote{If the objective value were negative, it would be best to not sample at all.}

%(i) queries the minimum number of softlabels from the teacher as possible to minimize computational and financial costs and (ii) ensure the obtained softlabels are accurate and not misleading for the student. 


==> Robust Active Distillation/sec/rad.tex <==
\section{Robust Active Distillation (RAD)}
\label{sec:rad}
%In this section, we motivate and present our approach, $\mathrm{RAD}$, that explicitly considers the competing objectives of efficiency and robustness in knowledge distillation.

\subsection{Background}
\label{sec:background-subsec}
The margin algorithm~\cite{liang2020mixkd,roth2006margin} selects the $b$ points with the lowest margin scores $\mathrm{margin}(x)$, where $b$ is our soft-label budget. Let $\margin$ be shorthand for the margin of each unlabeled input $\mathrm{margin}(x_i)$ and observe that its \emph{gain} or informativeness can be quantified as
$\gain = 1 - \margin$. Given a budget $b$, note that the margin-sampling algorithm corresponds to the optimal solution of the following optimization problem where the objective is to generate a probability distribution that maximizes the expected sum of gains,
\begin{equation}
\label{eqn:naive-max-gain}
\max \nolimits_{p \in \Delta_b} \E \nolimits_{\SS \sim p} \Big[\sum \nolimits_{i \in \SS} g_i\Big] \, \,  \text{, where } \Delta_b = \{p \in [0,1]^n: \sum \nolimits_{i \in [n]} p_i = b\}.
\end{equation}
As discussed previously, this formulation solely focuses on the informativeness of the points and does not consider the increased likelihood of mislabeling by the teacher.



\paragraph{Robust Distillation} To extend  \eqref{eqn:naive-max-gain} so that it is robust to possible teacher mislabeling, consider the masks
$
c_i = \1 \{\text{teacher labels point i correctly}\}$ for each $i \in [n]$
where $\1 \{x \} = 1$ if $x$ is true and 0 otherwise. Equipped with this additional variable, one way to
explicitly mitigate confirmation bias and simultaneously pick informative samples is to reward points that are correctly labeled by the teacher by assigning gains as before, but penalize those that are incorrectly labeled via losses. This can be done by using the modified gains in the context of \eqref{eqn:naive-max-gain}
$$
\tilde g_i = g_i c_i - (1 - c_i) \ell_i = \begin{cases}
g_i, &\text{ if teacher labels point i correctly} \\
-\ell_i, &\text{ otherwise }
\end{cases} \quad \forall{i \in [n]}.
$$
In words, this means that if the point $i$ is correctly labeled by the teacher we assign the standard margin-based gain $g_i = (1 - \margin)$ as before; otherwise, we penalize the selection by assigning $-\ell_i$ for some loss $\ell_i \ge 0$. This leads to the following general problem of robust distillation
\begin{equation}
    \label{prb:general}
    \max \nolimits_{p \in \Delta_b} \E \nolimits_{i \sim p} \left[g_i c_i - (1 - c_i) \ell_i \right].
\end{equation}


% \paragraph{Zero-loss Setting} For sake of simplicity, we assume henceforth that we are sampling a single point, i.e., $b = 1$. Setting the losses $\ell_i = 0$ for all $i \in [n]$ leads to the following modification of \eqref{eqn:naive-max-gain}
% \begin{equation}
% \label{eqn:max-gain-zero-loss}
% \max_{p \in \Delta_1} \E \nolimits_{i \sim p} \left[g_i c_i \right],
% \end{equation}
% which encourages the selection of points that are correctly labeled since picking an incorrect point does not contribute at all towards the gain. The formulation in \eqref{eqn:max-gain-zero-loss} encourages selecting instances that have high gains and are labeled correctly by the teacher, however, it does not at all account for the \emph{damage} that incorrectly labeled ones can have on the student. Prior work on confirmation bias has shown that even a small number misguided soft-labels can derail the student's performance and significantly impact its predictive capability~\cite{liu2021certainty}. Additionally, the harm of an incorrectly labeled point may be even more pronounced when the student is uncertain about that point. 
% %(i.e., high gain) about the data point to begin with. 

% \paragraph{Relative Loss} To overcome the limitations of the previous formulation, we consider instantiating the general framework \eqref{prb:general} with losses that are \emph{relative to the gain} $\ell_i = -w g_i$ for each $i \in [n]$ where $w \in [0,1]$ is a weight parameter that controls the magnitude of the penalization. This relative formulation purposefully leads to higher penalties misclassified points that the student is already unsure about (high gain) to mitigate confirmation bias, and leads to the following optimization problem which we consider in this paper
% \begin{equation}
% \label{prb:relative-ground-truth-prob}
% \max_{p \in \Delta_1} \E \nolimits_{i \sim p} \left[g_i c_i - (1 - c_i) w g_i \right].
% \end{equation}

The optimal solution to problem  \eqref{prb:general} corresponds to picking the $b$ most informative (highest gain) points \emph{among those that are predicted correctly by the teacher}, i.e., those points $i \in [n]$ with highest $g_i$ subject to $c_i = 1$. This approach is shown as  Robust Distillation (Oracle) in Fig.~\ref{fig:margin} (right). Fig.~\ref{fig:margin} exemplifies the effect of inaccurate examples on student training (see also ~\cite{pham2021meta}). If we had knowledge of $(c_i)_{i \in [n]}$, then we could optimally solve \eqref{prb:general} to obtain significant improvements over the standard margin algorithm. Unfortunately, perfect knowledge of whether the teacher labels each point correctly or not, i.e., $(c_i)_{i\in[n]}$, is not possible in the semi-supervised setting.


% \enote{I'm not sure yet, but consider moving this discussion elsewhere.} \cnote{I agree. I'm open to suggestions on where to place it} \cnote{Update: should this just be removed?}
% Given the success of the formulation with the indicator-modified gains, one lingering question is whether we can apply the same approach when we do not have access to the indicators $(c_i)_{i \in [n]}$. One approach is to use predict the masks using an algorithm like k-Nearest Neighbor (k-NN) with the gains as the input space. Here the k-NN can be constructed using a validation set of points with both the groundtruth label and the teacher's softmax label for each point and used to infer the indicators $(c_i)_{i \in [n]}$. However, as seen in Fig.~\ref{fig:margin}, even though the general trend is that low margin (high gain) points $i$are misclassified more often, it is very difficult to predict the indicator $c_i$ for each point $i$ \emph{individually}. In Sec.~\ref{sec:} of the appendix, we additionally describe our attempts at using k-NNs with various input spaces, ranging from the student's embedding layer to the input itself, to no avail.

\subsection{Our Approach}

We consider a general and robust approach that simultaneously leverages instance-specific knowledge without having to know the masks $(c_i)_{i\in [n]}$ individually. Suppose that we only know that the teacher mislabels $m$ points out of the $n$ unlabeled inputs $\XX_B$ instead. Can we generate a sampling distribution so that no matter which of the $m$ points are labeled incorrectly by the teacher, our expected gain is high? Assuming $b = 1$ for simplicity, we arrive at the extension of the formulation in \eqref{prb:general}
\begin{equation}
\label{prb:ours-general}
\max \nolimits_{p \in \Delta_1} 
\min \nolimits_{c\in\Delta_{n-m}}
%\E \nolimits_{i \sim p} \left[g_i c_i - (1 - c_i) w g_i \right],
\E \nolimits_{i \sim p} \left[g_i c_i - (1 - c_i) \ell_i \right], \text{where } \Delta_k = \{q \in [0,1]^n: \sum \nolimits_{i \in [n]} q_i = k\}.
\end{equation}


Problem~\eqref{prb:ours-general} has the following game theoretic interpretation. We go first and pick a sampling distribution $p$ over the points. In response, an adversary decides which points are misclassified (i.e, $c_i = 0$) by the teacher subject to the constraint that it can set $c_i = 0$ for at most $m \leq n$ of them since $c \in \Delta_{n-m}$. Given the linear structure of the problem, it turns out that we can invoke von Neumann's Minimax Theorem~\cite{neumann1928theorie} which states that the equilibrium point is the same regardless of whether we go first and pick the probability distribution $p \in \Delta_1$ or the adversary goes first and picks $(c_i)_{i \in [n]}$. By exploiting this connection, we obtain a closed form solution as formalized below.


\input{sec/proof_sketch}
\paragraph{RAD Loss} Equipped with Theorem~\ref{thm:minimax-max-gain}, all that remains is to specify the losses in~\eqref{prb:ours-general}. Prior work on confirmation bias has shown that even a small number misguided soft-labels can derail the student's performance and significantly impact its predictive capability~\cite{liu2021certainty}. Additionally, the harm of an incorrectly labeled point may be even more pronounced when the student is uncertain about that point. To model this, we consider instantiating our general problem formulation \eqref{prb:ours-general} with losses that are \emph{relative to the gain} $\ell_i = -w g_i$ for each $i \in [n]$ where $w \in [0,1]$ is a weight parameter that controls the magnitude of the penalization. This formulation purposefully leads to higher penalties for misclassified points that the student is already unsure about (high gain) to mitigate confirmation bias, and leads to the following optimization problem which is the focus of this paper
\begin{equation}
\label{prb:ours-negative}
\max \nolimits_{p \in \Delta_1} \min \nolimits_{c \in \Delta_{n-m}} \E \nolimits_{i \sim p} \left[g_i c_i - (1 - c_i) w g_i \right].
\end{equation}
Invoking Thm.~\ref{thm:minimax-max-gain} with the relative gain losses as described above immediately leads to the following, which, along with the choice of $w$ below, describes the algorithm \textsc{Rad} that we propose in this paper.
\begin{corollary}
\label{cor:negative}
An optimal solution $p^* \in \Delta_1$ to \eqref{prb:ours-negative} has $k$ non-zero entries $\II_{k^*} \subseteq [n]$ corresponding to the $k^*$ indices of the largest entries of $g$, with
$$
p^*_i = \frac{1}{g_i \sum_{j \in \II_{k^*}} g_j^{-1}} \quad \forall{i \in \II_{k^*}} \quad \text{where} \quad k^* = \argmax \nolimits_{k \in [n]} \frac{k - (1 + w)m}{ \sum_{j \in \II_k} g_j^{-1}}.
$$
The distribution $p^*$ can be computed in $\Theta(n \log n)$ time, with $\opt(k^*) = \nicefrac{(k^* - (1 + w)m)}{ \sum_{j \in \II_{k^*}} g_j^{-1}}$.
%$$\frac{k^* - (1 + w)m}{ \sum_{j \in \II_{k^*}} g_j^{-1}}.$$
\end{corollary} 
\rev{
\paragraph{Choice of $w$} Although \textsc{Rad} can be applied with any user-specified choice of $w$, we use the theoretically-motivated weight of $w = (1 - m/n)$ as the relative penalization constant in our experiments. This choice of $w$ guarantees that the optimal value (expected gain) of~\eqref{prb:ours-negative} (see Corollary~\eqref{cor:negative}) is non-negative --- if the expected gain were negative, we would be better off not sampling at all. \emph{This default value for $w$ makes \textsc{Rad} parameter-free.} Extensive empirical evaluations with varying values of $w$ are presented in  Sec.~\ref{sec:supp-robustness-w} of the Appendix.
}
%\textsc{Rad}'s robustness to the choice of $w$ and support the effectiveness of $w = 1 - m/n$ as the default value (see Sec.~\ref{sec:supp-robustness-w} of the Appendix).}

\begin{figure*}[ht!]
  \centering
  \begin{minipage}[t]{0.49\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/misc/teacher-gain.png}
  \end{minipage}%
  \hfill
  %\hspace{3px}
  \begin{minipage}[t]{0.49\textwidth}
  \centering
   \includegraphics[width=1\textwidth]{figs/misc/teacher-point-idx.png}
  \end{minipage}%

\caption{The optimal solution to \eqref{prb:ours-negative} given by Corollary~\ref{cor:negative} for various values for teacher accuracy (varying $m$). Even when most of the samples are labeled correctly by the teacher, our method is purposefully cautious and does not allocate all of the probability (of sampling) mass on the highest gain points.}
\label{fig:sampling-distribution}
\end{figure*}

We observe several favorable properties of \textsc{Rad}'s sampling distribution in Fig.~\ref{fig:sampling-distribution}, which depicts the computed distribution on a synthetic scenario with gains drawn uniformly at random from $[0,1]$.  For one, the sampling distribution tends to allocate less probability mass to the highest gain items. As prior work has shown, this is desirable because the hardest (highest gain) examples tend to be outliers or points with noisy labels~\citep{mindermann2022prioritized,ren2018learning}. In fact, robust learning approaches typically downweight hard examples for this reason~\cite{kumar2010self}, analogous to RAD's sampling behavior. At the same time, \citet{paul2021deep} show that the easiest (lowest gain) examples tend to be truly uninformative and the best strategy is to ignore a certain fraction of the highest and lowest gain points. This strategy parallels \textsc{Rad}'s computed distribution, where a number of low gain points are ignored and the probability peaks around a region inbetween (see Fig.~\ref{fig:sampling-distribution}). A prominent benefit of \textsc{Rad} is that this region is computed in a fully automated way as a function of the teacher's accuracy (i.e., amount of label noise). If the teacher is highly accurate, the distribution accordingly concentrates on the highest gain points (blue, Fig.~\ref{fig:sampling-distribution}); otherwise, it spreads out the probabilities over a larger portion of the points and purposefully assigns lower sampling probability to the highest gain points which are likely to be noisy (e.g., brown, Fig.~\ref{fig:sampling-distribution}).
%whereas it automatically spreads out the distribution and assigns a lower 
%In this regard, our formulation and analysis theoretically justify various heuristic thresholding schemes as a corollary~\cite{citovsky2021batch}.

%We observe that, contrary to standard margin, our sampling distribution tends to allocate less probability mass to the highest gain items. On the other hand, like standard margin, it completely avoids sampling (i.e., assigns $0$ probability to) a large portion of low-gain points based on a certain threshold that is a function of the teacher's accuracy (reliability). Notably, the optimal solution to \eqref{prb:ours-negative} is also reminiscent of a popular active learning strategy, where the top-$2b$ points with highest gain are selected and among them $b$ points are sampled uniformly at random~\cite{citovsky2021batch,balcan2007margin}. In this regard, our formulation and analysis leads to the theoretical justification of this scheme as a corollary. \cnote{TODO: elaborate on how this improves on and explains heuristics used in practice. See also~\cite{ren2018learning}}


\subsection{Implementation Details}
We conclude this section by outlining the practical details of \textsc{Rad}. \rev{We follow the setting of this section and set $\gain = 1 - \margin$ to define the gains of each point (see Sec.~\ref{sec:supp-robustness-gain} of the Appendix for evaluations with a differing gain definition).} In practice, we use the distribution $q = \min\{b p, 1\}$ when sampling a set of $b$ points, where $p$ is from Corollary~\ref{cor:negative}. This is optimal as long as the probabilities from Corollary~\ref{cor:negative} (or more generally, Theorem~\ref{thm:minimax-max-gain}) are not heavily concentrated on a few points (i.e., $\max_{i \in [n]} p_i \leq 1/b$). As exemplified in Fig.~\ref{fig:sampling-distribution} and experimentally verified in Sec.~\ref{sec:results} in all of the evaluated scenarios, we found this to virtually always be the case. Alternatively, the acquisition size $b$ can be adjusted after the single-sample probability distribution is computed so that $b \leq \min_{i \in [n]} 1 / p_i$. Since the number of mistakes the teacher makes on $\XX_B$, $m$, is not known to us in the semi-supervised setting, we approximate this quantity by first taking the sample mean inaccuracy of a small uniform random sample of $b_\mathrm{uniform}$ (see Appendix, Sec.~\ref{sec:supp-experimental-details}) points as a way to approximate $m$ and bootstrap our approach. We then use our approach with $b' = b - b_\mathrm{uniform}$ as described above. By Bernstein's inequality~\cite{bernstein1924modification}, this weighted estimate tightly concentrates around the mean, which in turn implies a high-quality approximation of $m$. We theoretically analyze the effect of an approximate $m$ on the quality of the optimal solution in Sec.~\ref{sec:supp-analysis} of the Appendix (see Lemmas~\ref{lem:supp-approx-m} and~\ref{lem:supp-estimating-m}). 

%(i) queries the minimum number of softlabels from the teacher as possible to minimize computational and financial costs and (ii) ensure the obtained softlabels are accurate and not misleading for the student. 


==> Robust Active Distillation/sec/related-work.tex <==
\section{Related Work}
\label{sec:related-work}

==> Robust Active Distillation/sec/reproducibility.tex <==
\section*{Reproducibility Statement}
Our algorithm is fully-specified (Corollary~\ref{cor:negative}), simple-to-implement, and parameter-free (Sec.~\ref{sec:rad}). We provide the full details and hyperparameters required to reproduce our results in Sec.~\ref{sec:results} and Sec.~\ref{sec:supp-experimental-details} of the Appendix. We specify descriptions of how the competing algorithms were implemented, including the hyperparameter settings. We provide precise theoretical results (Sec.~\ref{sec:rad} in the main body and Sec.~\ref{sec:supp-analysis} of the Appendix) that clearly specify the assumptions and provide full proofs and additional helper lemmas in the Appendix (Sec.~\ref{sec:supp-analysis}). Our evaluations use publicly available and easily accessible data sets and models.


% \paragraph{Ethics} Our work uses publicly available data sets and our contributions are mainly theoretical. 

==> Robust Active Distillation/sec/results.tex <==
\section{Results}
\label{sec:results}
We apply our sample selection algorithm, \textsc{Rad}, to benchmark vision data sets and evaluate its performance in generating high-performance student models on a diverse set of knowledge distillation scenarios. We compare the performance of \textsc{Rad} to the following: (i) \textsc{Margin}~\cite{balcan2007margin,roth2006margin} as described in Sec.~\ref{sec:rad}, (ii) \textsc{Uniform}, (iii) \textsc{Cluster Margin} (labeled \textsc{CM}), a state-of-the-art active learning technique~\cite{citovsky2021batch}, (iv) \textsc{Coreset}, a popular clustering-based active learning algorithm~\cite{sener2017active}, (v) \textsc{Entropy}, a greedy approach that picks the points with highest student prediction entropy~\cite{holub2008entropy}, and (vi) \textsc{UNIXKD}~\cite{xu2020computation}, a state-of-the-art active distillation approach based on mix-up~\cite{zhang2017mixup}. We implemented all algorithms in Python and used the TensorFlow~\cite{tensorflow2015-whitepaper} deep learning library. We used the hyperparameters specified in the respective papers for all of the compared approaches. For \textsc{Rad}, we use the theoretically-derived setting of $w = 1 - m/n$ as specified in Sec.~\ref{sec:rad} and emphasize that this makes \textsc{Rad} fully parameter-free. 
%We emphasize that \textsc{Rad} is fully parameter-free with the default $w = 1 - m/n$ (see Sec.~\ref{sec:rad}).

%

In Sec.~\ref{sec:supp-results} of the Appendix, we present: the full set of hyper-parameters and experimental details (Sec.~\ref{sec:supp-experimental-details}); additional evaluations that report statistics beyond test accuracy (Sec.~\ref{sec:supp-beyond-test-acc}); applications of \textsc{Rad} to the standard active learning setting and comparisons to SOTA approaches (Sec.~\ref{sec:supp-active-learning}); experiments with varying $w$ and gain definition to evaluate the robustness of \textsc{Rad} (Sec.~\ref{sec:supp-robustness-w} and~\ref{sec:supp-robustness-gain}, respectively); comparisons on a diverse set of knowledge distillation configurations (Sec.~\ref{sec:supp-varying-configurations}). Overall, our empirical evaluations show that \textsc{Rad} uniformly improves on state-of-the-art baselines and demonstrate its off-the-shelf effectiveness without the need to tune or change any hyperparameters.

%Additional experimental results that cover an even wider range of problem instances can be found in Sec.~\ref{sec:supp-results} of the Appendix.





\subsection{CIFAR10, CIFAR100, \& SVHN}
\paragraph{Setup} We use ResNet~\cite{resnet}, ResNetV2-$\{11, 20, 29\}$~\cite{resnetvtwo}, or MobileNet~\cite{mobilenet} with a depth multiplier of 1 as the student and ResNet-50, ResNetV2-$\{56, 110\}$, or MobileNet with a depth multiplier of 2 as the teacher model. We considered the CIFAR10/CIFAR100~\cite{cifar}, SVHN~\cite{svhn}, and ImageNet~\cite{imagenet} data sets. Unless otherwise specified, we use the Adam optimizer~\cite{kingma2014adam} with a batch size of $128$ with data set specific learning rate schedules. We follow the active distillation setting shown in Alg.~\ref{alg:active-distillation} with various configurations. We use 64 Cloud TPU v4s each with two cores.
%We considered a subsample of size $100$ to approximate the value of $m$ for \textsc{Rad} as specified by our analysis in Sec.~\ref{sec:supp-analysis} of the Appendix.
The full set of hyper-parameters and experimental details can be found in Sec.~\ref{sec:supp-results} of the Appendix.

\paragraph{Configurations} We experimented with a diverse set of configurations for the knowledge distillation task. We reported the specific configuration for each plot as part of the plot's title (e.g., see Fig.~\ref{fig:acc}). In context of the variables in the plot heading, we varied the number of epochs that the student is trained for (denoted as $e$), the size of the initial set of labeled points ($|A|$), the number of soft-labels to query per iteration ($b$), and the teacher model ($t$); \emph{resnet} in the configuration refers to ResNetV2-20 as the student and ResNet-50 as the teacher unless otherwise specified. All results were averaged over 10 trials unless otherwise stated. For each trial, we reshuffled the entire data set and picked a random portion (of size $|A|$) to be the labeled data set $\XX_L$, and considered the rest to be the unlabeled set $\XX_U$. 

\begin{figure*}[htb!]

%% FIRST ROW
    \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/resnets/1}
 %\subcaption{$$}
  \end{minipage}%
  \centering
  \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/resnets/2}
  \end{minipage}%
      \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/standard/11.png}
 %\subcaption{$$}
  \end{minipage}%
  \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/standard/2}
 %\subcaption{$$}
  \end{minipage}%
  
  %% SECOND ROW
        \begin{minipage}[t]{0.26\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/standard/3}
 %\subcaption{$$}
  \end{minipage}%
  \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/standard/4.png}
 %\subcaption{$$}
  \end{minipage}%
      \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/resnets/11}
 %\subcaption{$$}
  \end{minipage}%
  \centering
  \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/resnets/12}
  \end{minipage}%

  
  %% THIRD ROW
        \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/resnets/5.png}
 %\subcaption{$$}
  \end{minipage}%
  \centering
  \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/resnets/6.png}
  \end{minipage}%
      \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/standard/5.png}
 %\subcaption{$$}
  \end{minipage}%
  \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/standard/16.png}
 %\subcaption{$$}
  \end{minipage}%
  
  %% FOURTH ROW
        \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/standard/7.png}
 %\subcaption{$$}
  \end{minipage}%
  \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/standard/8.png}
 %\subcaption{$$}
  \end{minipage}%
          \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/resnets/7.png}
 %\subcaption{$$}
  \end{minipage}%
  \centering
  \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/resnets/8.png}
  \end{minipage}%

  
  %% FIFTH ROW
            \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/resnets/9.png}
 %\subcaption{$$}
  \end{minipage}%
  \centering
  \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/resnets/10.png}
  \end{minipage}%
      \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/standard/9.png}
 %\subcaption{$$}
  \end{minipage}%
  \begin{minipage}[t]{0.25\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/standard/10.png}
 %\subcaption{$$}
  \end{minipage}%

  % \textsc{Rad} consistently outperforms competing approaches in obtaining higher performing student models for a given teacher soft-labeling budget. 
		\caption{\rev{Evaluations of \textsc{Rad}, state-of-the-art active learning, and active distillation strategies on a diverse set of distillation configurations with varying data sets and network architectures. \textsc{Rad} consistently outperforms competing approaches. Shaded regions correspond to values within one standard deviation of the mean.}}
	\label{fig:acc}
% 	\vspace{-3ex}
\end{figure*}

In the first set of experiments, we evaluate the effectiveness of each method in generating high-accuracy student models subject to a soft-labeling budget on CIFAR10, CIFAR100, and SVHN data sets with ResNet(v2) and MobileNet architectures of varying sizes. CIFAR10 contains $50,000$ images of size $32\times 32$ with $10$ categories, CIFAR100 has $50,000$ $32\times 32$ images with $1000$ labels, and SVHN consists of $73,257$ real-world images ($32 \times 32$) taken from Google Street View. Fig.~\ref{fig:acc} depicts the results of our evaluations on a diverse set of knowledge distillation scenarios with varying configurations. We observe a consistent and marked improvement in the student model's predictive performance when our approach is used to actively select the points to be soft-labeled by the teacher. %The absolute increase in student accuracy when selecting points to soft-label by \textsc{Rad} can exceed $2\%$ in some scenarios.
This improvement is often present from the first labeling iteration and persists continuously over the active distillation iterations.

We observe that \textsc{Rad} performs particularly well relative to baselines regardless of the teacher's accuracy. For instance, we see significant improvements with \textsc{Rad} when distilling from a MobileNet teacher on CIFAR100, which has relatively low accuracy (see corresponding plots in Fig.~\ref{fig:acc}). This observation suggests that the explicit consideration of possible teacher inaccuracy is indeed helpful when distilling from a teacher that may be prone to making mistakes. At the same time, we observe that \textsc{Rad} outperforms state-of-the-art active learning algorithms such as Cluster Margin (CM) and others (\textsc{Margin}, \textsc{Entropy}) -- which do not explicitly consider label noise in the form of incorrect teacher soft-labels -- even in instances where the teacher accuracy is as high as $\approx 92\%$ (see SVHN plots in Fig.~\ref{fig:acc}). These observations support \textsc{Rad}'s ability to automatically adapt its sampling distribution to the applied scenario based on the approximated teacher inaccuracy.

% there are only a few incorrectly labeled points, e.g., on SVHN where the teacher's accuracy is $\approx90\%$. In fact, on SVHN the absolute improvement in test accuracy of the model generated by \textsc{Rad} is nearly $2\%$ relative to those of \textsc{Standard Margin} and \textsc{Uniform Sampling}.




\begin{figure*}[htb!]

  \centering
  
  \begin{minipage}[t]{0.34\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/imagenet/perf}
  \end{minipage}%
  %\hfill
  \begin{minipage}[t]{0.34\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/imagenet/trajectory}
  \end{minipage}%
  %\hfill
  \begin{minipage}[t]{0.34\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/imagenet/gain_updated}
 %\subcaption{$$}
  \end{minipage}%
		\caption{The classification accuracy and gain on the ImageNet data set with ResNets.}
	\label{fig:imagenet}
\end{figure*}


\subsection{ImageNet Experiments}
Here, we report the results of our evaluations with ResNet architectures trained on the ImageNet data set $I$, which contains nearly $1.3$ million images spanning $1000$ categories~\cite{imagenet}. We exclude the $\textsc{UnixKD}$ and $\textsc{Coreset}$ methods due to resource constraints and the fact that \textsc{CM} supersedes \textsc{Coreset}~\cite{citovsky2021batch} and \textsc{UnixKD} consistently performed poorly on the configurations in the previous subsection. This highlights an additional advantage of our approach: it merely requires a sort ($\Bigo(n \log n)$ total time). This is in contrast to computation- and memory-expensive methods like $\textsc{Coreset}$ and $\textsc{CM}$ that require clustering (see Sec.~\ref{sec:supp-imagenet} for details). Fig.~\ref{fig:imagenet} depicts the results of our evaluations, where our method consistently improves upon the compared approaches across all training epochs. Here the teacher is a ResNet50 model and the student is a ResNet18 model. The teacher is trained on the initial labeled dataset $A$ with $|A| = 10\%|I|$. For each choice of the budget $b \in \{3\%|I|, 5\%|I|, 7\%|I|, 9\%|I|, 11\%|I|\}$, we run $3$ trials.  In the rightmost plot we observe that the gain of our approach (w.r.t. $\gain = 1 - \margin$) is higher than that of the competing approaches, and that the gain correlates well with the test accuracy of the student, which reaffirms the practical validity of our formulation (Sec.~\ref{sec:rad}).

% \rev{
% \subsection{Discussion}
% % \subsection{Additional Comparisons with State-of-the-art}
% % In the previous subsections, our results indicated the improved performance of \textsc{Rad} over uniform sampling and standard margin sampling. Here, we present additional empirical comparisons to state-of-the-art active learning and active distillation techniques: \textsc{Cluster Margin}, a state-of-the-art active learning technique~\cite{citovsky2021batch}; \textsc{Coreset}, a popular clustering-based active learning algorithm~\cite{sener2017active}; \textsc{Entropy}-based uncertainty quantification~\cite{holub2008entropy}; and \textsc{UNIXKD}~\cite{xu2020computation}, a state-of-the-art active distillation approach based on mix-up~\cite{zhang2017mixup}. We used the suggested hyperparameters proposed in the respective papers for all of the compared approaches.

% Fig.~\ref{fig:comps-sota} shows the results of our comparisons. From the figures, we see that \textsc{Rad} outperforms the competing approaches, including UNIXKD, an algorithm that is specifically designed for the active distillation scenario. We conjecture that these results are explained by the presence of multiple hyperparameters of existing approaches, which makes them brittle to varying problem instances. This is in contrast to \textsc{Rad}'s favorable empirical performance that comes with theoretical guarantees. Moreover, unlike the compared approaches, \textsc{Rad} is fully parameter-free and runs in near linear time ($\mathcal{O}(n \log n)$). %These simultaneous favorable properties are in contrast to those of the competing approaches.
% %For instance, clustering-based approaches like \textsc{Coreset} require $\mathcal{O}(n d b)$ time for approximate clustering, where $d$ is the dimension of the embedding layer and $b$ is the sample size.


% \begin{figure*}[htb!]

%   \centering
  
%   \begin{minipage}[t]{0.33\textwidth}
%   \centering
%  \includegraphics[width=1\textwidth]{figs/sota/resnet29-on-svhn(e=100,_A_=10000,b=1000,t=resnet56).png}
%   \end{minipage}%
%   %\hfill
%   \begin{minipage}[t]{0.33\textwidth}
%   \centering
% \includegraphics[width=1\textwidth]{figs/sota/resnet20-on-cifar100(e=100,_A_=20000,b=5000,t=resnet56).png}
%   \end{minipage}%
%   %\hfill
%   \begin{minipage}[t]{0.33\textwidth}
%   \centering
%  \includegraphics[width=1\textwidth]{figs/sota/resnet29-on-svhn(e=100,_A_=5000,b=1000,t=resnet101).png}
%  %\subcaption{$$}
%   \end{minipage}%
% 		\caption{\rev{Comparisons to state-of-the-art active learning and active distillation strategies. Overall, \textsc{Rad} consistently leads to improved distillation performance over benchmarks.}}
% 	\label{fig:comps-sota}
% \end{figure*}





%\subsection{Discussion}




==> sec/analysis.tex <==
\section{Analysis}
\label{sec:analysis}

We assume throughout that $\nnz{g} > m$ so that the optimal objective value of \eqref{eqn:problem} is strictly positive. 
\begin{lemma}
An optimal solution $p^* \in \Delta$ to \eqref{eqn:problem} has $k$ non-zero entries $\II_k \subseteq [n]$ corresponding to the $k$ indices of the largest entries of $g$, with
$$
p^*_i = \frac{1}{g_i \sum_{j \in \II_k} g_j^{-1}} \quad \forall{i \in \II_k},
$$
with objective value
$$
\frac{k - m}{ \sum_{j \in \II_k} g_j^{-1}}.
$$
The distribution $p^*$ can be computed in $\Theta(n \log n)$ time.
\end{lemma} 
\begin{proof}
Let $p$ be an optimal solution to \eqref{eqn:problem} and WLOG assume that $p_1 g_1 \ge p_2 g_2 \ge \cdots p_n g_n$. Let $k = \nnz{p}$ and define $S(p, g) = \sum_{i = m+1}^k p_i g_i$. Note that 
$$
S(p, g) = \min_{c \in \{0, 1\}^n: \dotp{c}{\mathbf{1}} = n - m} \E \nolimits_{i \sim p}[g_i c_i]
$$
since the adversary would select $c$ to remove the top $m$ highest entries of $p g$.

Let $w = p_{m+1} g_{m+1}$. By optimality of $p$, it must be that $p_1 g_1 = \cdots = p_{m+1} g_{m+1} = w$. Otherwise, we could increase the value of $p_{m+1} g_{m+1}$ by removing probability mass from $p_1, \ldots, p_m$ and increasing $p_{m+1}$ accordingly until $pg$ is equal in the first $m+1$ entries, which would lead to a higher objective value.

We now claim that in fact $p_1 g_1 = \cdots = p_k g_k$ for some optimal $p$. Suppose this does not hold, i.e., the equality in probability-weighted gains are not equal for all optimal solutions.  optimal solution $p$ smallest index $j > m+1$ for which $p_j g_j < w$. Construct a new probability distribution $p'$ by scaling up the probabilities $p_j, \ldots, p_k$ by $\alpha > 1$ and scaling down $p_1, \ldots, p_{j-1}$ by $\beta \in (0,1)$ until $p_j g_j$ matches the rescaled $w$, i.e., $\alpha p_j g_j = \beta w = \beta p_{m+1} g_{m+1}$. The values for $\alpha$ and $\beta$ that lead to such a probability distribution are
$$
\alpha = \frac{w}{(1 - z) p_j g_j + z w} \quad \text{and} \quad \beta = 1 - \frac{z(\alpha - 1)}{1 - z},
$$
where $z = \sum_{i = j}^k p_i$. Note that $p'$ is indeed a valid distribution since the sum is equal to 1 and none of the increased probabilities exceed 1\footnote{Since $
\alpha p_i = \frac{w p_i}{(1 - z) p_j g_j + z w} \leq \frac{zw}{(1 - z) p_j g_j + z w} \leq 1
$ for all $i = j, \ldots, k$.}.


Define $S_1 = \sum_{i=j}^{k} p_i g_i$ and $S_2 = \sum_{i=1}^{j-1} p_i g_i$ and note that $S(p, g) = S_1 + S_2$. Similarly, for $p'$ defined as the rescaled distribution above, we have $S(p', g) = \alpha S_1 + \beta S_2$. We now compare $S(p', g)$ and $S(p, g)$:
\begin{align*}
    S(p', g) - S(p, g) &= \alpha S_1 + \beta S_2 - (S_1 + S_2) \\
    %&= (\alpha - 1) S_1 - \frac{z(\alpha - 1) S_2}{1 - z} \\
    &= (\alpha - 1) \left(S_1 - \frac{z}{1-z} S_2\right).
\end{align*}
It follows that $(\alpha - 1) > 0$ by definition, so the quantity above is strictly positive if $S_1 > \frac{z}{1-z} S_2$. By the optimality of $p$, we know that it is better to have the entries of $j, \ldots, k$ to be non-zero. This means that if we were to set $p_j, \ldots, p_k$ to 0 and increase the probabilities $p_1, \ldots, p_{j-1}$ by a factor of $(1 - z)^{-1}$, we would have a lower objective value\footnote{If the objective values are equal, then we are done since the altered probability distribution is an optimal solution with $j$ non-zero entries $p_1 g_1 = \cdots = p_j g_j$.}.
%\footnote{If the objective value is the same, i.e., if $p$ is not a unique solution, then we can recurse on this argument by starting from the rescaled distribution with $p_j, \ldots, p_k = 0$ until an optimal solution with fewer nonzero entries is not possible.}
$$
S_1 + S_2 > \frac{S_2}{1-z}.
$$
Rearranging, this implies that $S_1 > z/(1-z) S_2$, and from the calculations above, that
$$
S(p', g) - S(p, g) > 0,
$$
which contradicts the optimality of $p$. This proves that the optimal distribution $p$ must satisfy 
$$
p_{i} g_{i} = p_{j} g_{j} \quad \forall{i, j \in \nz{p}},
$$
where $\nz{p} = \{i \in [n] : p_i > 0 \}$.

To complete the proof, note that the above means that the optimal distribution $p$ must have the form
\begin{equation}
\label{eqn:closed-form}
p_i = \frac{1}{g_i \sum_{j \in \nz{p}} g_j^{-1}} \quad \forall{i \in \nz{p}},
\end{equation}
with the objective value 
\begin{equation}
\label{eqn:obj-val}
\frac{|\nz{p}| - m}{\sum_{j \in \nz{p}} g_j^{-1}}.
\end{equation}
For a fixed $\nnz{p}$, the above is maximized whenever $\sum_{j \in \nz{p}} g_j^{-1}$ is minimized, which occurs when the indices of non-zero probabilities $\nz{p}$ correspond to the top-$|\nz{p}|$ gains. The optimal distribution can be generated as follows. First, we sort the gains in descending order $g_1 \ge g_2 \ge \cdots \ge g_n$ and pre-compute the cumulative histogram for $\sum_{j =1}^k g_j^{-1}$ for each $k \in [n]$. This takes $\Theta(n \log n)$ time. Then, we generate $\nz{p}$ by picking the $k \in [n]$ that maximizes \eqref{eqn:obj-val}. This takes $\Theta(n)$ time, for a total of $\Theta(n \log n)$ time to generate $p^*$.

% At each iteration $i \in [n]$, we check whether setting the $i^\text{th}$ index as in Eq.~\ref{eqn:closed-form} would lead to an increase in the objective value and if so, we set it accordingly, otherwise we stop and return the probability vector. From the objective value above, we see that the stopping condition occurs when
% $$
% \frac{|\nz{p}| + 1 - m}{\sum_{j \in \nz{p}} g_j^{-1} + g_i^{-1}} < \frac{|\nz{p}| - m}{\sum_{j \in \nz{p}} g_j^{-1}}
% $$
\end{proof}

\subsection{Batch-based Formulation}
\newtheorem{observation}[theorem]{Observation}
\begin{observation}[Diminishing returns]
The rate of gain $r_i$ of each bucket $i \in [t]$ is monotonically decreasing with the amount of mass allotted to it, i.e.,
$r_i(x) \leq r_i(y)$ for $x \ge y$.
\end{observation}

\begin{lemma}[Monotonicity of optimal allocation]
Let $\AA^*(b) = (b_1, ..., b_t)$ with $\sum_{i=1}^t \AA_i^*(b) = b$ be the optimal allocation with respect to budget b. For any $b' \geq b$, we have that $\AA^*_i(b) \leq \AA^*_i(b')$ for all $i \in [t]$.
\end{lemma}
\begin{proof}
Suppose there exists $i \in [t]$ such that $\AA^*_i(b) > \AA^*_i(b')$. This implies that there must exist a $j \in [t]$ such that $\AA^*_j(b) < \AA^*_j(b')$ with 
\begin{equation}
\label{eqn:exists}
r_i(\AA^*_i(b')) < r_j(\AA^*_j(b') - \epsilon)
\end{equation}
for all $\epsilon \in (0, \AA^*_j(b')]$. But, by Observation 1 and the fact that $\AA^*_i(b)$ is optimal for budget $b$, we observe a contradiction for $\epsilon = \min\{\AA^*_i(b) - \AA^*_i(b'),\AA^*_j(b') - \AA^*_j(b)\}$:
\begin{align*}
r_i(\AA^*_i(b')) &\ge r_i(\AA^*_i(b) - \epsilon) &\text{by Observation 1 since $\AA^*_i(b') \leq \AA^*_i(b) - \epsilon$} \\
&\ge r_j(\AA^*_j(b)) &\text{By optimality of $\AA^*(b)$}\\
&\ge r_j(\AA^*_j(b') - \epsilon) &\text{by Observation 1 since $\AA^*_j(b) \leq \AA^*_j(b') - \epsilon$} \\
&> r_i(\AA^*_i(b')) &\text{by \eqref{eqn:exists}},
\end{align*}
and this establishes the lemma.
\end{proof}

==> sec/minimax.tex <==

% \section{Proof for relative penalties}
% \enote{This should be replaced with the previous section, ``Proof for general penalties.''}

% \begin{lemma}
% \label{lem:minimax-max-gain-old}
% Let $n > m$ be integers, together with weight $w \ge 0$, such that $n-m(1+w) \ge 0$.
% Let $f(p, c) = \sum_i g_i p_i c_i - \sum_i w g_i p_i (1-c_i)$, and let $\Delta_{\ell} = \{ x\in [0, 1]^n : \sum_i x_i = \ell \}$.
% Then we can find an optimal solution $p^* \in \Delta_1$ to 
% $\argmax_{p \in\Delta_1} min_{c\in\Delta_{n-m}} f(p,c)$ in linear time, assuming we are given $g_i$ in sorted order, i.e. $g_1 \geq g_2 \geq g_3 \geq \ldots \geq g_n$.

% Define $H_k = \sum_{i \leq k} 1/g_i$, and
% let $N(k) = (k - m(1+w)) / H_k$. Then the solution is given by
% $$
% k^* = \argmax_{k\ge m(1+w)} N(k)
% $$
% and
% \begin{align*}
% p_i^* 
%     =&
%         \frac{1}{g_i H_{k^*}} \mbox{\ \ if $i \leq k^*$}
%         \mbox{\ \ and $p_i^*=0$ otherwise.}
% \end{align*}
% The maximum value $\min_{c\in\Delta_{n-m}} f(p^*, c)$ is $N(k^*)$.
% \end{lemma} 
% \begin{proof}
% Our proof relies on the the Minimax Theorem~\cite{neumann1928theorie}, which yields
% $$
% \min_{c\in\Delta_{n-m}} \max_{p\in\Delta_1} f(p,c) = \max_{p\in\Delta_1} \min_{c\in\Delta_{n-m}} f(p,c).
% $$

% Before beginning, we will first simplify $f(p,c)$ somewhat, finding
% \begin{align*}
% f(p, c) 
%     =& \sum_i g_i p_i c_i - \sum_i w g_i p_i (1-c_i)\\
%     =& \sum_i (c_i(1+w) - w) g_i p_i
% \end{align*}

% Now, consider the value $\min_{c\in\Delta_{n-m}} f(p^*, c)$, where $p^*$ is defined as in the lemma's statement. Notice that $g_i p_i^* = 1 / H_{k^*}$ for $i\leq k^*$, and 0 otherwise.
% Substituting, we see
% \begin{align*}
% f(p^*, c)
%     =& \sum_i (c_i(1+w) - w) g_i p^*_i \\
%     =& \sum_{i\leq k^*} (c_i(1+w) - w) / H_{k^*} \\
%     =& \frac{1+w}{ H_{k^*}} \sum_{i\leq k^*} c_i - k^*\frac{w}{ H_{k^*}}
% \end{align*}
% Clearly, this is minimized by making $c_i = 1$ for all $i>k^*$, leaving
% $\sum_{i\leq k^*} c_i = k^*-m$. Hence,
% \begin{align*}
% \min_{c\in\Delta_{n-m}} f(p^*, c)
%     =& \frac{1+w}{ H_{k^*}} (k^*-m) - k^*\frac{w}{ H_{k^*}} \\
%     =& \frac{k^*-m(1+w)}{ H_{k^*}} = N(k^*)
% \end{align*}
% This does not yet prove that $p^*$ is optimal, but it does show that
% $$
% N(k^*) = \min_{c\in\Delta_{n-m}} f(p^*, c)
%     \leq \max_{p\in\Delta_1} \min_{c\in\Delta_{n-m}} f(p, c)
% $$

% To show optimality, we'll provide a choice for $c$, denoted $c^*$, and show that $\max_{p\in\Delta_1} f(p, c^*) = N(k^*)$. Combined with the Minimax Theorem, this will be enough to complete the proof.

% To this end, define
% \begin{align*}
% c^*_i =& \begin{cases}
%     \frac{1}{1+w} \left( N(k^*)/g_i + w \right) \mbox{\ \ if $i\leq k^*$}    \\
%     1 \mbox{\ \ otherwise}
%     \end{cases}
% \end{align*}
% Notice that $\sum_i c^*_i = n - m$. Further,
% $c_i^*(1+w) - w = N(k^*)/g_i$ for $i\leq k^*$, and 1 otherwise.
% Substituting, we see
% \begin{align*}
% f(p, c^*)
%     =& \sum_i (c_i(1+w) - w) g_i p_i \\
%     =& \sum_{i\leq k^*} N(k^*) p_i + \sum_{i> k^*} g_i p_i 
% \end{align*}
% Before continuing, we observe that $N(k^*) \ge g_i$ for $i> k^*$. (To see this, we'll use the easy-to-prove rule that $\frac{a}{b} \geq \frac{a+c}{b+d}$ implies $\frac{a}{b} \geq \frac{c}{d}$ for positive numbers. The observation then follows since $N(k^*) \ge N(k^*+1)$, where $N(k^*) = \frac{k-m(1+w)}{H_{k^*}}$ and
% $N(k^*+1) = \frac{k-m(1+w) + 1}{H_{k^*} + 1/g_{k^*+1}}$.)

% So, $f(p, c^*)$ is maximized when $p_i = 0$ for $i > k^*$. Since $\sum_i p_i = 1$, we see $\max_{p\in\Delta_1} f(p, c^*) = N(k^*) \geq \min_{c\in\Delta_{n-m}} \max_{p\in\Delta_1} f(p, c)$. Applying Minimax and our earlier result, we have
% \begin{align*}
% N(k^*) = \min_{c\in\Delta_{n-m}} f(p^*, c)
%     \leq \max_{p\in\Delta_1} \min_{c\in\Delta_{n-m}} f(p, c)
%     = \min_{c\in\Delta_{n-m}} \max_{p\in\Delta_1} f(p, c)
%     \leq N(k^*)
% \end{align*}
% That is, $p^*$ attains the maximum value, as we wanted.
% \end{proof}


% \ignore{
% \subsection{Graveyard}

% \begin{align*}
% N(k^*) &\geq N(k^*+1) \\
% \frac{k-M}{H_{k^*}} &\geq \frac{k-M+1}{H_{k^*} + 1/g_{k^*+1}}\\
% (k-M)(H_{k^*} + 1/g_{k^*}) & \geq (k-M + 1) H_{k^*} \\
% (k-M)/g_{k^*} &\geq H_{k^*} \\
% N(k^*) &\geq g_{k^*}
% \end{align*}
% }  %% end ignore

==> sec/prefix.tex <==

\section{Proof for prefix with general penalties}

\begin{lemma}
\label{lem:minimax-max-gain}
Given $g_1 \geq g_2 \geq g_3 \geq \ldots \geq g_n > 0$ and $\ell_i \ge 0$ for $i\in\{1, 2, \ldots, n\}$, let
$f(p, c) = \sum_i g_i p_i (1-c_i) - \sum_i \ell_i p_i c_i$. Also let
$G_k = \sum_{i\leq k} \frac{g_i}{g_i+\ell_i}$ and 
$H_k = \sum_{i\leq k} \frac{1}{g_i+\ell_i}$.

Let $\gamma:\{1, 2, \ldots, n\} \rightarrow \mathbb{R}$ be an increasing function, and define
\begin{align*}
\Delta_{\gamma} = \{ x\in [0, 1]^n : \forall_k, \sum_{i\le k} x_i \leq \gamma(k) \}
\end{align*}
(We write $\Delta_1 = \{ x\in [0, 1]^n : \forall_k, \sum_{i\le k} x_i \leq 1 \} = \{ x\in [0, 1]^n : \sum_{i\le n} x_i \leq 1 \}$.)
Suppose $G_n \geq \gamma(n)$.
Then we can find an optimal solution $p^* \in \Delta_1$ to 
$\argmax_{p \in\Delta_1} min_{c\in\Delta_\gamma} f(p,c)$ in linear time.
 
The solution is given by
$$
k^* = \argmax_{k\ge m} \frac{G_k - \gamma(k)}{H_k}
$$
and
\begin{align*}
p_i^* 
    =&
        \frac{1}{H_{k^*}(g_i+\ell_i)} \mbox{\ \ if $i \leq k^*$}
        \mbox{\ \ and $p_i^*=0$ otherwise.}
\end{align*}
The maximum value $\min_{c\in\Delta_\gamma} f(p^*, c)$ is $N(k^*)$, where $N(k)$ is defined to be $\frac{G_k-\gamma(k)}{H_k}$.
\end{lemma} 
\begin{proof}
The proof relies on the the Minimax Theorem~\cite{neumann1928theorie}, which yields
$$
\min_{c\in\Delta_\gamma} \max_{p\in\Delta_1} f(p,c) = \max_{p\in\Delta_1} \min_{c\in\Delta_\gamma} f(p,c).
$$
We will further use two claims, which we'll prove shortly.

\begin{Claim}\label{claim:p}
Let $p^*$, $k^*$, and $N(k)$ be defined as in the statement of the lemma. Then $p^*\in\Delta_1$ and $N(k^*) = \min_{c\in\Delta_\gamma} f(p^*, c)$.
\end{Claim}

\begin{Claim}\label{claim:c}
Let $k^*$ and $N(k)$ be defined as in the statement of the lemma. Further, define
\begin{align*}
c^*_i =& 
    \max\left(0, \frac{g_i - N(k^*)}{g_i + \ell_i}\right)
\end{align*}
Then $c^*\in\Delta_\gamma$ and
$N(k^*) = \max_{p\in\Delta_1} f(p, c^*)$.
\end{Claim}
Given the claims, we see
\begin{align*}
N(k^*) = \min_{c\in\Delta_\gamma} f(p^*, c) 
    \leq& \max_{p\in\Delta_1} \min_{c\in\Delta_\gamma} f(p, c) \mbox{\ \ by Claim~\ref{claim:p}} \\
    =& \min_{c\in\Delta_\gamma}\max_{p\in\Delta_1} f(p, c) \mbox{\ \ by Minimax} \\
    \leq& \max_{p\in\Delta_1} f(p, c^*) = N(k^*) \mbox{\ \ by Claim~\ref{claim:c}}
\end{align*}
That is, $p^*$ attains the maximum, which is $N(k^*)$, as we wanted.

We now prove the claims.
Before beginning, we will first simplify $f(p,c)$ somewhat, finding
\begin{align*}
f(p, c) 
    =& \sum_i g_i p_i(1- c_i) - \sum_i \ell_i p_i c_i\\
    =& \sum_i (g_i - c_i(g_i + \ell_i)) p_i
\end{align*}
\begin{proof}[Proof of Claim~\ref{claim:p}]
We first show $p^*\in\Delta_1$. We have
\begin{align*}
\sum_{i\leq n} p^*_i = \sum_{i\leq k^*} p^*_i 
    = \sum_{i\leq k^*} \frac{1}{H_{k^*}(g_i+\ell_i)} 
    = \frac{H_{k^*}}{H_{k^*}} = 1
\end{align*}
And since $p^*_i \ge 0$ for all $i$, it immediately follows that $p^*_i \leq 1$ as well.

We now show $N(k^*) = \min_{c\in\Delta_{n-m}} f(p^*, c)$. To this end,
\begin{align*}
f(p^*, c)
    =& \sum_{i\leq n} (g_i - c_i(g_i + \ell_i)) p_i \\
    =& \sum_{i\leq k^*} \frac{g_i - c_i(g_i + \ell_i)}{H_{k^*}(g_i+\ell_i)} \\
    =& \sum_{i\leq k^*} \frac{g_i}{H_{k^*}(g_i+\ell_i)} -
    \sum_{i\leq k^*} \frac{c_i} {H_{k^*}} \\
    =&  \frac{G_{k^*}}{H_{k^*}} -
   \frac{1} {H_{k^*}}  \sum_{i\leq k^*} c^*_i
\end{align*}
Clearly, for $c^*\in\Delta_\gamma$, this expression is minimized when $\sum_{i\leq k^*} c_i = \gamma(k^*)$.
\enote{We need a little more here. Basically, we want to set $c_i = 1$ for $i\in [k^*-\gamma(k^*)+1, k^*]$ and $c_i =0$ otherwise. So long $\gamma$ allows this, we're happy. Otherwise, things get weird.}
So we have
\begin{align*}
\min_{c\in\Delta_\gamma} f(p^*, c)
    &= \frac{G_{k^*}}{H_{k^*}} -\frac{\gamma(k^*)} {H_{k^*}}
    = N(k^*)
\end{align*}
as claimed.
\end{proof}

We now prove our second claim.
\begin{proof}[Proof of Claim~\ref{claim:c}]
We first show that $N(k^*) \ge g_i$ for $i>k^*$.\footnote{In the border case that $k^*=n$, we can add a dummy item with $g_{n+1}=0$ and the claim follows trivially.}
Observe that if $\frac{a}{b} \ge \frac{a+c}{b+d}$, then $\frac{a}{b} \ge \frac{c}{d}$ for non-negative values (and $b>0, d>0$).
Notice
\begin{align*}
\frac{G_{k^*}-m}{H_{k^*}} = N(k^*)\ge  
N(k^*+1) =\frac{G_{k^*}+g_{k^*+1}/(g_{k^*+1}+\ell_{k^*+1})-m}{H_{k^*}+1/(g_{k^*+1}+\ell_{k^*+1})} 
\end{align*}
By our observation,
$$
N(k^*) \ge \frac{g_{k^*+1}/(g_{k^*+1}+\ell_{k^*+1})}{1/(g_{k^*+1}+\ell_{k^*+1})} = g_{k^*+1} \ge g_i \mbox{\ \ for $i>k^*$.}
$$
Similarly, we show $N(k^*) \le g_i$ for $i\leq k^*$, using the observation that if $\frac{a-c}{b-d} \leq \frac{a}{b}$, then $\frac{a}{b} \le \frac{c}{d}$ for non-negative values (and $b-d>0$ and $d>0$).
Notice
\begin{align*}
N(k^*-1) = 
\frac{G_{k^*}-g_{k^*}/(g_{k^*}+\ell_{k^*})-m}{H_{k^*}-1/(g_{k^*}+\ell_{k^*})} 
\leq \frac{G_{k^*}-m}{H_{k^*}}
= N(k^*)
\end{align*}
And again, by our observation,
$$
N(k^*) \le \frac{g_{k^*}/(g_{k^*}+\ell_{k^*})}{1/(g_{k^*}+\ell_{k^*})} = g_{k^*} \le g_i \mbox{\ \ for $i\le k^*$.}
$$
Now we're ready to prove the claim.

We first show $c^*\in\Delta_{n-m}$. Since $N(k^*) \le g_i$ for $i\le k^*$, we see
$c^*_i = \frac{N(k^*)+\ell_i}{g_i + \ell_i} \le 1$ for $i\le k^*$. So $c^*_i \in [0, 1]$. Further,
\begin{align*}
\sum_{i\le n} c^*_i
    =& \sum_{i\le k^*} \frac{N(k^*)+\ell_i}{g_i + \ell_i} + \sum_{k^* < i \le n} 1 \\
    =& \sum_{i\le k^*} \frac{N(k^*)-g_i}{g_i + \ell_i} + \sum_{i\le k^*}\frac{g_i+\ell_i}{g_i + \ell_i}  +\sum_{k^* < i \le n} 1 \\
    =& N(k^*) H_{k^*} - G_{k^*} + n \\
    =& G_{k^*} - m - G_{k^*} + n = n-m
\end{align*}
That is, $c^*\in\Delta_{n-m}$.

Finally, we show $N(k^*) = \max_{p\in\Delta_1} f(p, c^*)$. Note that 
$c^*_i(g_i+\ell_i) - \ell_i = N(k^*)$
for $i\le k^*$, while 
$c^*_i(g_i+\ell_i) - \ell_i = g_i$ for $i> k^*$.
We have
\begin{align*}
f(p, c^*) 
    =& \sum_i (c^*_i(g_i + \ell_i) - \ell_i) p_i\\
    =& \sum_{i\leq k^*} N(k^*) p_i
        +\sum_{i> k^*} g_i p_i
\end{align*}
From above, $N(k^*) \ge g_i$ for $i>k^*$. So the expression is maximized for $p\in\Delta_1$ when $p_i = 0$ for $i> k^*$ and $\sum_{i\leq k^*} p_i = 1$. Hence,
\begin{align*}
\max_{p\in\Delta_1} f(p, c^*) = N(k^*)
\end{align*}
as we wanted.
\end{proof} %% End proof of claim.
\end{proof} %% End proof of lemma.


\ignore{
\subsection{Graveyard}

\begin{align*}
N(k^*) &\geq N(k^*+1) \\
\frac{k-M}{H_{k^*}} &\geq \frac{k-M+1}{H_{k^*} + 1/g_{k^*+1}}\\
(k-M)(H_{k^*} + 1/g_{k^*}) & \geq (k-M + 1) H_{k^*} \\
(k-M)/g_{k^*} &\geq H_{k^*} \\
N(k^*) &\geq g_{k^*}
\end{align*}
}  %% end ignore

==> sec/rad-old-good-state.tex <==
\section{Robust Active Distillation (RAD)}
\label{sec:rad}
In this section, we motivate and present our approach, $\mathrm{RAD}$, that explicitly considers the competing objectives of efficiency and robustness in knowledge distillation.

\subsection{Problem Statement}

Recall that the margin algorithm~\cite{liang2020mixkd,roth2006margin} selects the $b$ points with the lowest margin scores $\mathrm{margin}(x)$, where $b$ is our soft-label budget. Let $\margin$ be shorthand for the margin of each unlabeled input $\mathrm{margin}(x_i)$ and observe that its \emph{gain} or informativeness can be quantified as
$$
\gain = (1 - \margin).
$$
Given a budget $b$, note that the margin-sampling algorithm corresponds to the optimal solution of the following optimization problem where the objective is to generate a probability distribution that maximizes the sum of gains,
\begin{equation}
\label{eqn:naive-max-gain}
\max_{p \in \Delta_b} \E_{\SS \sim p} \Big[\sum_{i \in \SS} g_i\Big] \, \,  \text{, where } \Delta_b = \{p \in [0,1]^n: \sum_{i \in [n]} p_i = b\}.
\end{equation}
As discussed previously. this formulation solely focused on the informativeness of the points and does not consider the increased likelihood of mislabeling by the teacher.



\paragraph{Robust Distillation} To extend  \eqref{eqn:naive-max-gain} so that it considers robustness, consider the masks
$$
c_i = \1 \{\text{teacher labels point i correctly}\} \quad \forall{i \in [n]},
$$
where $\1 \{x \} = 1$ if $x$ is true and 0 otherwise. Equipped with this additional variable, one way to
explicitly mitigate confirmation bias and simultaneously pick informative samples is to reward points that are correctly labeled by the teacher by assigning gains as before, but penalize those that are incorrectly labeled via losses. This can be done by using the modified gains in the context of \eqref{eqn:naive-max-gain}
$$
\tilde g_i = g_i c_i - (1 - c_i) \ell_i = \begin{cases}
g_i, &\text{ if teacher labels point i correctly} \\
-\ell_i, &\text{ otherwise }
\end{cases} \quad \forall{i \in [n]}.
$$
In words, this means that if the point $i$ is correctly labeled by the teacher we assign the standard margin-based gain $g_i = (1 - \margin)$ as before; otherwise, we penalize the selection by assigning $-\ell_i$ for some loss $\ell_i \ge 0$. This leads to the following general problem of robust distillation
\begin{equation}
    \label{prb:general}
    \max_{p \in \Delta_1} \E \nolimits_{i \sim p} \left[g_i c_i - (1 - c_i) \ell_i \right].
\end{equation}


\paragraph{Zero-loss Setting} For sake of simplicity, we assume henceforth that we are sampling a single point, i.e., $b = 1$. Setting the losses $\ell_i = 0$ for all $i \in [n]$ leads to the following modification of \eqref{eqn:naive-max-gain}
\begin{equation}
\label{eqn:max-gain-zero-loss}
\max_{p \in \Delta_1} \E \nolimits_{i \sim p} \left[g_i c_i \right],
\end{equation}
which encourages the selection of points that are correctly labeled since picking an incorrect point does not contribute at all towards the gain. The formulation in \eqref{eqn:max-gain-zero-loss} encourages selecting instances that have high gains and are labeled correctly by the teacher, however, it does not at all account for the \emph{damage} that incorrectly labeled ones can have on the student. Prior work on confirmation bias has shown that even a small number misguided soft-labels can derail the student's performance and significantly impact its predictive capability~\cite{liu2021certainty}. Additionally, the harm of an incorrectly labeled point may be even more pronounced when the student is uncertain about that point. 
%(i.e., high gain) about the data point to begin with. 

\paragraph{Relative Loss} To overcome the limitations of the previous formulation, we consider instantiating the general framework \eqref{prb:general} with losses that are \emph{relative to the gain} $\ell_i = -w g_i$ for each $i \in [n]$ where $w \in [0,1]$ is a weight parameter that controls the magnitude of the penalization. This relative formulation purposefully leads to higher penalties misclassified points that the student is already unsure about (high gain) to mitigate confirmation bias, and leads to the following optimization problem which we consider in this paper
\begin{equation}
\label{prb:relative-ground-truth-prob}
\max_{p \in \Delta_1} \E \nolimits_{i \sim p} \left[g_i c_i - (1 - c_i) w g_i \right].
\end{equation}

The optimal solution to problem  \eqref{prb:relative-ground-truth-prob} corresponds to picking the most informative (highest gain) points \emph{among those that are predicted correctly by the teacher}, i.e., those points $i \in [n]$ with highest $g_i$ subject to $c_i = 1$. This approach is shown as  Robust Distillation (Oracle) in Fig.~\ref{fig:margin} (right). As Fig.~\ref{fig:margin} and our additional results in Sec.~\ref{sec:supp-results} of the Appendix consistently show, if we have knowledge of $(c_i)_{i \in [n]}$, then we can optimally solve \eqref{prb:relative-ground-truth-prob} above to obtain significant improvements over the standard margin algorithm. Unfortunately, however, perfect knowledge of whether the teacher labels a point correctly or not, i.e., $(c_i)_{i\in[n]}$, is never possible in the semi-supervised learning setting.


% \enote{I'm not sure yet, but consider moving this discussion elsewhere.} \cnote{I agree. I'm open to suggestions on where to place it} \cnote{Update: should this just be removed?}
% Given the success of the formulation with the indicator-modified gains, one lingering question is whether we can apply the same approach when we do not have access to the indicators $(c_i)_{i \in [n]}$. One approach is to use predict the masks using an algorithm like k-Nearest Neighbor (k-NN) with the gains as the input space. Here the k-NN can be constructed using a validation set of points with both the groundtruth label and the teacher's softmax label for each point and used to infer the indicators $(c_i)_{i \in [n]}$. However, as seen in Fig.~\ref{fig:margin}, even though the general trend is that low margin (high gain) points $i$are misclassified more often, it is very difficult to predict the indicator $c_i$ for each point $i$ \emph{individually}. In Sec.~\ref{sec:} of the appendix, we additionally describe our attempts at using k-NNs with various input spaces, ranging from the student's embedding layer to the input itself, to no avail.

\subsection{Our Approach}

%\enote{Again, I'm not sure. This description saves space, and might be easier to understand for readers. Breaking it into (1) no penalty, then (2) penalty proportional to $wg_i$ tells a better story.} 
%\cnote{Done. Please let me know if this is the structure you had in mind.}
%% \enote{looks good. commenting out the notes}
We consider a general and robust approach that simultaneously leverages instance-specific knowledge without having to know the masks $(c_i)_{i\in [n]}$ individually. Suppose that we only knew that the teacher mislabels $m$ points out of the $n$ unlabeled inputs $\XX_B$. Can we generate a sampling distribution so that no matter which of the $m$ points are labeled incorrectly by the teacher, our expected gain is high? Assuming for simplicity that $b = 1$, this question leads to the following which extends \eqref{prb:relative-ground-truth-prob}
\begin{equation}
\label{prb:ours}
\max_{p \in \Delta_1} 
%\min_{c \in \{0, 1\}^n: \dotp{c}{\mathbf{1}} = n - m} 
\min_{c\in\Delta_{n-m}}
\E \nolimits_{i \sim p} \left[g_i c_i - (1 - c_i) w g_i \right],
\end{equation}
where $\Delta_k = \{q \in [0,1]^n: \sum_{i \in [n]} q_i = k\}$ as before. 

Problem~\eqref{prb:ours} has the following game theoretic interpretation. We go first and pick a sampling distribution $p$ over the points $n$. In response, an adversary decides which points are misclassified by the teacher subject to the constraint that it can set $c_i = 0$ for (i.e., misclassify) at most $m \leq n$ of them since $c \in \Delta_{n-m}$. By von Neumann's Minimax Theorem~\cite{neumann1928theorie} the objective value is the same regardless of whether we go first and pick the probability distribution or the adversary goes first and picks $(c_i)_{i \in [n]}$. In fact, it turns out that this observation applies to the analogue of the more general framework formulation~\eqref{prb:general} with arbitrary gains and losses, and this connection leads to a closed form solution for the optimal distribution as formalized in the theorem below.


\begin{figure*}[ht!]
  \centering
  \begin{minipage}[t]{0.49\textwidth}
  \centering
 \includegraphics[width=1\textwidth]{figs/misc/teacher-gain.png}
  \end{minipage}%
  \hfill
  %\hspace{3px}
  \begin{minipage}[t]{0.49\textwidth}
  \centering
   \includegraphics[width=1\textwidth]{figs/misc/teacher-point-idx.png}
  \end{minipage}%

\caption{The optimal solution to \eqref{prb:ours} given by Lemma~\ref{lem:single-sample-lemma} for various values for teacher accuracy (varying $m$). Even when most of the samples are labeled correctly by the teacher, our method is purposefully cautious and does not allocate all of the probability (of sampling) mass on the highest gain points.}
\label{fig:sampling-distribution}
\end{figure*}

\input{sec/proof_sketch}

\ignore{
\begin{lemma}
\label{lem:single-sample-lemma}
An optimal solution $p^* \in \Delta_1$ to \eqref{prb:ours} has $k$ non-zero entries $\II_{k^*} \subseteq [n]$ corresponding to the $k^*$ indices of the largest entries of $g$, with
$$
p^*_i = \frac{1}{g_i \sum_{j \in \II_{k^*}} g_j^{-1}} \quad \forall{i \in \II_{k^*}} \quad \text{where} \quad k^* = \argmax_{k \in [n]} \frac{k - (1 + w)m}{ \sum_{j \in \II_k} g_j^{-1}}.
$$
The distribution $p^*$ can be computed in $\Theta(n \log n)$ time and achieves an objective value of
$$\frac{k^* - (1 + w)m}{ \sum_{j \in \II_{k^*}} g_j^{-1}}.$$
\end{lemma} 
\begin{proof}
\enote{proof sketch} \cnote{Should the proof sketch be for the more general lemma in the appendix? But in that case maybe that doesn't belong in the proof of this lemma, since we are just applying Lemma~\ref{lem:minimax-max-gain} with $\ell_i = w g_i$ here}
Let $G(p, c) = \E \nolimits_{i \sim p} \left[g_i c_i - (1 - c_i) w g_i \right]$. By linearity of $G(p, c)$ and integrality of $n - m$ the minimum over the masks $c$ is attained at the boundary points, i.e.,
$$
\min_{c \in \{0, 1\}^n: \dotp{c}{\mathbf{1}}  = n - m} G(p, c) = \min_{c \in \Delta_{n-m}} G(p, c) \quad \forall{p \in \Delta_1}.
$$
This form now allows us to invoke von Neumann's Minimax Theorem~\cite{neumann1928theorie} to show that the optimal solution $p^*$ given above attains the optimal objective value. This is formalized in Lemma~\ref{lem:minimax-max-gain} of the Appendix and its application leads to the lemma statement.
\end{proof}
}


Fig.~\ref{fig:sampling-distribution} depicts examples of the optimal solution on a synthetic scenario with gains drawn uniformly at random from $[0,1]$. We observe that, contrary to the standard margin, our sampling distribution tends to allocate less probability mass to the highest gain items. On the other hand, like standard margin, it completely avoids sampling (i.e., assigns $0$ probability to) a large portion of low-gain points based on a certain threshold that is a function of the teacher's accuracy (reliability). Notably, the optimal solution to \eqref{prb:ours} is also reminiscent of a popular active learning heuristic, where the top-$2b$ points with highest gain are selected and among them $b$ points are sampled uniformly at random. In this regard, our formulation and analysis leads to its theoretical justification as a byproduct~\cite{citovsky2021batch}.


\subsection{Implementation Details}
We conclude this section by outlining the practical details of \textsc{Rad}. In particular, we detail the procedure used to sample a batch of points, approximate the value of $m$, and set the weight parameter $w$ in the context of \eqref{prb:ours}. In practice, we use the distribution $q = \min\{b p, 1\}$ when sampling a set of $b$ points, where $p$ is from Lemma~\ref{lem:single-sample-lemma}. This is optimal as long as the probabilities from Lemma~\ref{lem:single-sample-lemma} are not heavily concentrated on a few points (i.e., $\max_{i \in [n]} p_i \leq 1/b$). As exemplified in Fig.~\ref{fig:sampling-distribution} and experimentally verified in Sec.~\ref{sec:results} in all of the evaluated scenarios, we found this to always be the case. Alternatively, the acquisition size $b$ can be adjusted after the single-sample probability distribution is computed so that $b \leq \min_{i \in [n]} 1 / p_i$.
 
 Since the number of mistakes the teacher makes on $\XX_B$, $m$, is not known to us in the semi-supervised setting, we approximate this quantity by first taking the sample mean inaccuracy of a small uniform random sample of $b_\mathrm{uniform}$ points as a way to approximate $m$ and bootstrap our approach. We then use our approach with $b' = b - b_\mathrm{uniform}$ (i.e., $q = \min\{b' p, 1\}$) as described above. By Bernstein's inequality~\cite{bernstein1924modification}, this weighted estimate tightly concentrates around the mean, which in turn implies a high-quality approximation of $m$. The details of this procedure and the effect of using an approximate value of $m$ on the quality of the optimal solution to \eqref{prb:ours} are discussed in Sec.~\ref{sec:supp-analysis} of the Appendix. Finally, we use the weight $w = (1 - m/n)$ as the relative penalization constant. This choice of $w$ ensures that the optimal value of~\ref{prb:ours} as specified by Lemma~\ref{lem:single-sample-lemma} is non-negative (and in fact, proportional to $(n - m)^2/n$), which justifies the sampling procedure in the first place.\footnote{If the objective value were negative, it would be best to not sample at all.}

%(i) queries the minimum number of softlabels from the teacher as possible to minimize computational and financial costs and (ii) ensure the obtained softlabels are accurate and not misleading for the student. 


==> sec/related-work.tex <==
\section{Related Work}
\label{sec:related-work}
